QueenV2: Future of Quantum Circuit Simulation

A state vector-based quantum circuit simulation can provide accurate results for the development and validation of quantum computing algorithms, without being affected by noise interference. However, existing quantum circuit simulators have consistently underperformed due to inadequate integration with quantum circuits and high-performance computing architectures. To tackle the challenges in quantum computing, we propose QueenV2, which builds upon the design principles of Queen and elevates performance to a new level. Experimental results on the NVIDIA RTX-4090 demonstrate that QueenV2 achieves up to a 40x improvement in gate performance and a 5x improvement in circuit performance compared to hyQuas. Furthermore, QueenV2 realizes a 137x speedup in gate benchmarks and a 14x speedup in circuit performance relative to NVIDIA cuQuantum, enabled by gate fusion via the IBM Qiskit toolkit. By eliminating reliance on third-party libraries, QueenV2 is positioned to significantly accelerate quantum circuit simulation, thus promoting the development of innovative accelerators and quantum algorithms.

==> contents/AD.tex <==
\section{Artifact Evaluation (AD)}
\subsection{Paper's Main Contributions}
\begin{description}
\item [$C_1$] This paper introduces an all-in-one optimization module designed to convert original quantum circuits into optimized versions that are more tailored for execution on classical computers.
\item [$C_2$] This paper presents the implementation and performance analysis of the all-in-cache simulation module with a high-speed simulation workflow.
\item[$C_3$] This paper conducts a comparative analysis of simulation performance utilizing qubit, gate, and circuit benchmarks on multi-GPUs against state-of-the-art simulators.
\end{description}

\subsection{Computational Artifacts}
To safeguard against unauthorized use, please email to the authors.

\begin{center}
\begin{tabular}{rll}
\toprule
Artifact ID  &  Contributions &  Related \\
             &  Supported     &  Paper Elements \\
\midrule
$A_1$ & $C_1$ & Figure 5 \\
\midrule
$A_2$ & $C_2$, $C_3$ & Figure 8 \\
& & Figure 9 \\
& & Figure 10 \\
& & Figure 11 \\
& & Figure 12 \\
%\midrule
\bottomrule
\end{tabular}
\end{center}

\begin{center}
    \textbf{\noindent{Artifact Identification}}
\end{center}

\subsection{Computational Artifact A1}
\noindent\textit{Relation To Contributions}

This artifact $A_1$ is an implementation of $C_1$, which is an optimization tool for doing the qubit reordering and gate fusion within the quantum circuits.

\noindent\textit{Expected Results}

This artifact aims to transform any circuits (e.g., QFT, QAOA, or BV) into the optimized circuit file, which includes gate blocks, in-memory swapping (SQS), and cross-device swapping (CSQS).
Specifically, the input format for the circuit is structured as follows.
\begin{center}
\begin{tcolorbox}[breakable]
\textbf{[Gate type] \textcolor{red}{[Target qubits]} [ID] [Remain info]}
\end{tcolorbox}
\end{center}

Given an example circuit represented in Figure 5 (a), along with our specified input format, the optimization module is capable of producing the optimized circuit as output.
\begin{center}
\begin{tcolorbox}[breakable]
\textbf{H \textcolor{red}{0} 0}
\\\textbf{ H \textcolor{red}{1} 1}
\\\textbf{ RZZ \textcolor{red}{2 4} 2}
\\\textbf{ RZZ \textcolor{red}{5 7} 3}
\\\textbf{ H \textcolor{red}{8} 4}
\\\textbf{ H \textcolor{red}{9} 5}
\\\textbf{ H \textcolor{red}{3} 6}
\\\textbf{ H \textcolor{red}{6} 7}
\\\textbf{ RZZ \textcolor{red}{0 2} 8}
\\\textbf{ RZZ \textcolor{red}{4 7} 9}
\\\textbf{ H \textcolor{red}{9} 10}
\\\textbf{ RZZ \textcolor{red}{1 8} 11}
\\\textbf{ RZZ \textcolor{red}{3 6} 12}
\\\textbf{ H \textcolor{red}{5} 13}
\end{tcolorbox}
\end{center}

The output resulting from the qubit reordering optimization should match Figure 5(b) as follows.
The target qubit for each original gate operation should not exceed the chunk size of 4, which is also marked in red.
\begin{center}
\begin{tcolorbox}[breakable]
\textbf{3} \textcolor{ForestGreen}{\# Gate Block Size}
\\\textbf{H \textcolor{red}{0} 0}
\\\textbf{H \textcolor{red}{1} 1}
\\\textbf{H \textcolor{red}{3} 6}
\\\textbf{1}
\\\textbf{SQS 3 0 1 3 4 5 7} \textcolor{ForestGreen}{\# In-memory swapping}
\\\textbf{4}
\\\textbf{RZZ \textcolor{red}{0 2} 2}
\\\textbf{RZZ \textcolor{red}{1 3} 3}
\\\textbf{RZZ \textcolor{red}{0 3} 9}
\\\textbf{H \textcolor{red}{1} 13}
\\\textbf{1}
\\\textbf{SQS 3 0 1 3 4 6 7}
\\\textbf{3}
\\\textbf{H \textcolor{red}{1} 7}
\\\textbf{RZZ \textcolor{red}{1 3} 12}
\\\textbf{RZZ \textcolor{red}{0 2} 8}
\\\textbf{1}
\\\textbf{SQS 2 0 2 6 7}
\\\textbf{1}
\\\textbf{CSQS 2 6 7 8 9} \textcolor{ForestGreen}{\# Cross-device swapping}
\\\textbf{1}
\\\textbf{SQS 2 0 2 6 7}
\\\textbf{1}
\\\textbf{SQS 1 3 5}
\\\textbf{4}
\\\textbf{H \textcolor{red}{2} 5}
\\\textbf{H \textcolor{red}{2} 10}
\\\textbf{H \textcolor{red}{0} 4}
\\\textbf{RZZ \textcolor{red}{0 3} 11}
\end{tcolorbox}
\end{center}

After applying all features in this module, the result should match Figure 5(c). The diagonal gates, such as RZZ, within each gate block, will be merged without altering correctness.
To avoid excessive elaboration, detailed results are not provided.
Please verify this matter effortlessly through the scripts we provided.

To verify the optimized circuit executes in the correct sequence and with proper dependencies
on target qubits, one can utilize our validation script as follows.
\begin{center}
\begin{tcolorbox}[breakable,colback=blue!5!white,colframe=blue!75!black]
\textbf{\$ }\textcolor{ForestGreen}{\# switch workspace to the validation directory}
\\
\textbf{\$ cd ./tests}
\\
\textbf{\$ }\textcolor{ForestGreen}{\# run the validation script}
\\
\textbf{\$ ./validate\_circuit\_order.sh}
\end{tcolorbox}
\end{center}


If all optimized circuits have the correct sequence, the message "Passed all circuit order validations" will be output to the terminal. Otherwise, a mismatch error will be invoked.

\noindent\textit{Expected Reproduction Time (in Minutes)}
% \artexpl{
% Estimate the time required to reproduce the artifact, providing separate estimates for the individual steps: Artifact Setup, Artifact Execution, and Artifact Analysis.
% }

The expected results of this module are listed as follows.
\begin{easylist}
& The required time for Artifact Setup is negligible if our provided raw circuit file is adopted. Otherwise, installing the Python package of the open-source project may take 5-10 minutes.
& For Artifact Execution, each optimized circuit of our benchmark is consistently generated within 0.5 seconds.
& For Artifact Analysis, the optimized circuit does not represent the actual simulation efficiency, so we refrain from discussing it for now.
\end{easylist}

\noindent\textit{Artifact Setup (incl. Inputs)}

\textit{Hardware:} No specific Hardware is required to execute the experiments.

\textit{Operating System:} We employ Docker with Ubuntu 22.04 and kernel version 5.15.0-1044-nvidia for our experiments. However, no specific operating system is required to execute the experiments.

\textit{Software:} No specific software is required to execute the experiments.
However, for the convenience of downloading the open-source circuit generator and facilitating subsequent simulation stages, we still recommend installing all necessary environments at this stage.

\begin{easylist}
& In order to generate highly reproducible circuits in an open-source manner and facilitate direct comparisons with various works in one single execution environment, Python 3.10.12 should be used along with the following package dependencies. (i.e., using different configurations does not ensure running the experiments for all related works in one single environment):
    && attrs==20.3.0
    && cachetools==5.3.3
    && certifi==2021.5.30
    && charset-normalizer==3.3.2
    && cirq==0.13.1
    && cirq-aqt==0.13.1
    && cirq-core==0.13.1
    && cirq-google==0.13.1
    && cirq-ionq==0.13.1
    && cirq-pasqal==0.13.1
    && cirq-rigetti==0.13.1
    && cirq-web==0.13.1
    && contourpy==1.2.0
    && cuquantum-cu12==23.10.0
    && custatevec-cu12==1.5.0
    && cutensor-cu12==1.7.0
    && cutensornet-cu12==2.3.0
    && cycler==0.12.1
    && decorator==5.1.1
    && dill==0.3.8
    && duet==0.2.9
    && fonttools==4.49.0
    && google-api-core==1.34.1
    && google-auth==2.28.2
    && googleapis-common-protos==1.63.0
    && grpcio==1.62.1
    && grpcio-status==1.48.2
    && h11==0.9.0
    && httpcore==0.11.1
    && httpx==0.15.5
    && idna==2.10
    && iso8601==0.1.16
    && kiwisolver==1.4.5
    && lark==0.11.3
    && matplotlib==3.8.3
    && mpmath==1.3.0
    && msgpack==1.0.8
    && networkx==2.8.8
    && numpy==1.26.4
    && nvidia-cublas-cu12==12.3.4.1
    && nvidia-cuda-runtime-cu12==12.3.101
    && nvidia-cusolver-cu12==11.5.4.101
    && nvidia-cusparse-cu12==12.2.0.103
    && nvidia-nvjitlink-cu12==12.3.101
    && packaging==24.0
    && pandas==2.2.1
    && pbr==6.0.0
    && pillow==10.2.0
    && ply==3.11
    && protobuf==3.20.3
    && psutil==5.9.8
    && py==1.11.0
    && pyasn1==0.5.1
    && pyasn1-modules==0.3.0
    && pydantic==1.8.2
    && PyJWT==1.7.1
    && pyparsing==3.1.2
    && pyquil==3.0.1
    && python-dateutil==2.8.2
    && python-rapidjson==1.16
    && pytz==2024.1
    && pyzmq==25.1.2
    && qcs-api-client==0.8.0
    && qiskit==0.46.0
    && qiskit-aer-gpu==0.13.3
    && qiskit-terra==0.46.0
    && requests==2.31.0
    && retry==0.9.2
    && retrying==1.3.4
    && rfc3339==6.2
    && rfc3986==1.5.0
    && rpcq==3.11.0
    && rsa==4.9
    && ruamel.yaml==0.18.6
    && ruamel.yaml.clib==0.2.8
    && rustworkx==0.14.2
    && scipy==1.12.0
    && six==1.16.0
    && sniffio==1.2.0
    && sortedcontainers==2.4.0
    && stevedore==5.2.0
    && symengine==0.11.0
    && sympy==1.12
    && toml==0.10.2
    && tqdm==4.66.2
    && typing\_extensions==4.10.0
    && tzdata==2024.1
    && urllib3==2.2.1
\end{easylist}

\textit{Datasets / Inputs:} To lessen the load on users for recompilation, the experimental inputs consist of a designated configuration file and a total of 17 distinct gates and circuits, accessible via the ./circuit directory.
Alternatively, one can also generate all the raw circuits with the following command.

\begin{center}
\begin{tcolorbox}[breakable,colback=blue!5!white,colframe=blue!100!black]
\textbf{\$ }\textcolor{ForestGreen}{\# install required packages listed in the \emph{Software} section}
\\
\textbf{\$ pip3 install -r requirements.txt}
\\
\textbf{\$ }\textcolor{ForestGreen}{\# switch workspace to the following directory}
\\
\textbf{\$ cd ./optimizer}
\\
\textbf{\$ }\textcolor{ForestGreen}{\# generate raw circuits (e.g., BV, QAOA, ..., etc) }
\\
\textbf{\$ ./gen\_raw\_circuits.sh}
\\
\end{tcolorbox}
\end{center}

\textit{Installation and Deployment:}
The version of the GNU g++ compiler used is 11.04.

\noindent\textit{Artifact Execution}
A workflow may consist of two tasks: $T_1$ and $T_2$.
Task $T_1$ compiles the C++ source code for the all-in-one module.
Task $T_2$ leverages the module to transform the raw circuits in all experiments into optimized circuits.
The dependency of tasks is $T_1 \rightarrow T_2$
Note that the raw circuits have already been obtained in the \emph{dataset/input} section.

\noindent\textit{Artifact Analysis (incl. Outputs)}
In terms of efficiency, the elapsed time for transforming any raw circuit is less than 1 second on a DGX-A100, thanks to the polynomial-time complexity of the implementation.

Moreover, this artifact demonstrates promising results in reducing the number of gate blocks.
For example, the 31-qubit QFT circuit with 496 gates is grouped into only 18 gate blocks.
Theoretically, memory access time could be reduced by a factor of 27 (496/18). However, in practice, this reduction is usually unattainable due to considerations involving compiler optimizations, making it more of a reference point.

The reductions in gate blocks result in fewer in-memory swaps and cross-device swaps compared to other works, thereby enhancing an 8-fold times speedup while running the circuit through our simulation module ($A_2$) on the DGX-A100, a significance that is elaborated upon in more depth in the AE.

\subsection{Computational Artifact A2}
\noindent\textit{Relation To Contributions}

This artifact $A_2$ is a comprehensive tool for quantum circuit simulation that orchestrates the complete implementation of $C_2$.
%Running this artifact with a performance profiler yields the results of $C_3$ on the given machines.
The integration of various benchmarks and other simulators can showcase the efficiency of $C_3$ (i.e., demonstrating higher efficiency compared to the other works).
Alongside the generated circuit via artifact $A_1$, this stage enables the presentation of a comprehensive performance report.

\noindent\textit{Expected Results}

The expected results of each benchmark on a DGX-A100 workstation are listed as follows.
These benchmarking results can dominate state vector-based simulation in various cases, as mentioned in 

\begin{easylist}
& QAOA Benchmark: \\Our work with fusion should get a performance improvement of 4.x compared to cuQuantum and aer with gate fusion, and our work in a single GPU without fusion still outperforms Aer and cuQuantum with fusion in 2 GPUs.
& QFT Benchmark: \\Our work with fusion should get a performance improvement of 4.x compared to cuQuantum and aer with gate fusion, and our work in a single GPU without fusion still outperforms Aer and cuQuantum with fusion in 2 GPUs.
& Qubit Benchmark: \\Our work should get an average performance improvement of 9.x compared to cuQuantum and Aer in various qubit scenarios.
& Strong Scaling Benchmark: \\This experiment demonstrates that our work has strong scaling capability, achieving an average performance improvement of 8.7x compared to cuQuantum and Aer in various device scenarios.
& Gate Benchmark: \\ To show the versatility of various gates, our work should get an average performance improvement of 8.7x compared to cuQuantum and Aer.
& Circuit Benchmark: \\To show the versatility of various circuits, our work should get an average performance improvement of 9.x compared to cuQuantum and Aer.
& Breakdown of 34-qubit Simulation Time: \\Gate operation should occupy the most time. This experiment can be used to analyze the whole simulation process for different circuits.
& Breakdown of 34-qubit Simulation Time w/o NVLink and shared memory: \\The cross-device swapping should occupy the most time. This experiment serves as a benchmark for comparison against NVLink and socket-based methodologies.
& Roofline Model of The 30-qubit H-gate Benchmark: \\Our work should be computation-bound, while QuEST should be memory-bound, highlighting the decisive difference that demonstrates us as the next-generation simulator.
\end{easylist}

\arttime

\begin{easylist}
& For Artifact Setup, the required time is negligible if our Dockerfile is adopted. 
Otherwise, installing the NVIDIA Driver, CUDA toolkit, and NCCL library may take up to 30 minutes, depending on network speed.

& For Artifact Execution, we provide the expected computational time of this artifact on a DGX-A100 as follows.
Notably, the proficiency with which information is gathered using a profiler varies depending on the familiarity with the operations.
    && QAOA Benchmark: 16 minutes
    && QFT Benchmark: 5 minutes
    && Qubit Benchmark: 4 minutes
    && Strong Scaling Benchmark: 3 minutes
    && Gate Benchmark: 15 minutes
    && Circuit Benchmark: 15 minutes
    && Breakdown of 34-qubit Simulation Time: 15 minutes
    && Breakdown of 34-qubit Simulation Time without NVLink: 150 minutes
    && Roofline Model: 3 minutes
& For Artifact Analysis, the required time is negligible when utilizing our provided script, which summarizes the results into a CSV and PDF file for each experiment.
%Otherwise, each experiment may take 5-10 minutes to discern the parameters and input for various simulators.
\end{easylist}

\artin

\artinpart{Hardware}

For the experiments, we use a DGX-A100 workstation comprising two AMD EPYC 7742 CPUs and eight NVIDIA A100 SXM GPUs interconnected via NVLink, boasting a bandwidth of 600GB/s.

\artinpart{Operating System}
We employ Docker with Ubuntu 22.04 and kernel version 5.15.0-1044-nvidia for our experiments. 
However, no specific operating system is required to execute the experiments.

\artinpart{Software}
We use NVCC ver. 12.3.107 and the NCCL library ver. 2.20.3.
To reproduce the related works, the Python environment matches that of artifact $A_1$. You also need cmake to build QuEST, the related work we compared our work against. The version of cmake we use is ver. 3.22.1.

\artinpart{Datasets / Inputs}
All circuit inputs can be obtained after completing the steps of artifact $A_1$.

\artinpart{Installation and Deployment}

For compilation, we use NVCC ver. 12.3.107 with the "-lnccl -arch=sm\_80 -O3 
-{}- jump-table-density=0 -maxrregcount=64" flags and the NCCL library ver. 2.20.3 for compiling the CUDA codes.

To compile the executable file, execute "make -j" in the terminal within the ./simulator directory of the workspace path, and no specific requirements for deploying our work.

To execute the experiments, ensure the configure and circuit files exist, then run it with the following suggested command.
\begin{center}
\begin{tcolorbox}[breakable,colback=blue!5!white,colframe=blue!100!black]
\textbf{\$ ./simulator/Quokka -i [configure file] -c [circuit file]}
\end{tcolorbox}
\end{center}

\artcomp

A workflow may consist of three tasks: $T_1$, and $T_2$.
The task $T_1$ generates specific configure files, quantum gates, and circuits as benchmarks with optimizations for the simulators\footnote{The task $T_1$ represents the entire process of artifact $A_1$. If already completed, please skip this step.
}.
These configurations and benchmarks are then used as input by computational task $T_2$.
The outputs can be directly displayed in the terminal.
The results can also be automatically summarized as a CSV and PDF file if one utilizes our provided scripts.
%With a comprehensive chart or additional plotting package in task $T_3$, exquisite performance reports can be presented.
The dependencies for reproducing our work are as follows: $T_1 \rightarrow T_2$.
The detailed step-by-step reproduction will be detailed in the Artifact Evaluation section.

The details of the experimental parameters are listed as follows.
\begin{easylist}
& In our simulator, specifying the size of the simulated qubits is achieved by switching the configuration file. This can be done by modifying the value of N in the .ini file.
& In our simulator, simulating different circuits only requires switching the .txt file without the need for recompilation.
Rest assured, our scripts, codes with comments, and README.md files offer abundant examples to aid in completing all experiments.
& The default number of qubits in the A100 scenario is set to 31 (this is the memory upper limit), but please adjust it according to your GPUs.
& There are 7 practical quantum circuits and 10 standard quantum gates used as benchmarks. 
You can still generate specific simulation circuit files according to your needs, but please refer to the advanced user manual to complete this task.
& Given that the circuits executed in benchmarks and simulated scenarios are both large-scale, it is recommended to run the simulations multiple times to remove noise, even though running once is usually sufficient to indicate the simulation time.
\end{easylist}



Overall, we utilize the better elapsed time to identify a more effective simulation result.
A brief analysis and interpretation of each benchmark are listed below.
\begin{easylist}
& QAOA Benchmark:
\\This benchmark evaluates the overall simulation with gate fusion on a specific 31-qubit QAOA circuit.
Our work with gate fusion gets the fastest results on a DGX-A100.
& QFT Benchmark: 
\\This benchmark evaluates the overall simulation with gate fusion on a specific 31-qubit QFT circuit.
Our work with gate fusion gets the fastest results on a DGX-A100.
& Qubit Benchmark:
\\This benchmark evaluates the time per gate for the standard Hadamard gate with qubits ranging from 24 to 31.
It demonstrates the performance of the simulator under varying memory consumption levels.
Our work gets the fastest results for all cases on an A100.
& Strong scaling Benchmark:
\\This benchmark evaluates the time per gate for the standard Hadamard gate with devices ranging from 1 to 8 exponentially.
It demonstrates the robust scalability of the simulator under varying GPU devices.
Our work gets the fastest results for all cases on a DGX-A100.
& Gate benchmark:
\\This benchmark evaluates the time per gate for different types of gates on a 31-qubit system.
It demonstrates the high performance of each implementation for all varying gates.
Our work gets the fastest results for all cases on an A100.
& Circuit benchmark:
\\This benchmark evaluates the time per gate for different types of practical circuits on a 31-qubit system.
It demonstrates the high performance of each implementation for varying circuits.
Our work gets the fastest results for all cases on an A100.
& Breakdown of 34-qubit simulation time:
\\This hotspot analysis demonstrates the elapsed times of different techniques, providing insight into the performance bottlenecks of different models, with NVLink serving as the transfer medium for cross-device communication.
Observing the changes in elapsed time, it can be noted that introducing in-memory swapping and cross-device swapping is highly beneficial.
& Breakdown of 34-qubit simulation time without NVLink and shared memory:
\\This hotspot analysis demonstrates the elapsed times of different techniques, providing insight into the performance bottlenecks of different models without relying on NVLink for cross-device communication. Observing the changes in elapsed time, it can be noted that utilizing NVLink for cross-device swapping is highly beneficial.
& Roofline model of the 30-qubit H-gate benchmark: \
\\This analysis is typically used to determine whether the application is computation-bound or memory-bound.
By utilizing the Nsight Compute profiler, it is evident that our simulator is computation-bound across different levels of GPU.
For other simulators (we take QuEST as an example), the performance is significantly limited by memory bandwidth.
\end{easylist}

==> contents/ADAE.tex <==
\twocolumn[%
{\begin{center}
\Huge
Appendix: Artifact Description/Artifact Evaluation        
\end{center}}
]

\apppart{Reproducibility}
Unlike other claimed state-of-the-art simulators, this work can be reliably reproduced using the artifact description and artifact evaluation provided.
You are welcome to challenge our simulator performance or play with us.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  AD Appendix
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\appendixAD

\section{Overview of Contributions and Artifacts}

\subsection{Paper's Main Contributions}

%\artexpl{ Provide a list of all main contributions of the paper.}

% \artsampl{
% \begin{description}
% \item[$C_1$] This is the 1st contribution.
% \item[$C_2$] This is the 2nd contribution.
% \item[$C_3$] This is the 3rd contribution.
% \end{description}
% }

\begin{description}
\item [$C_1$] This paper introduces an all-in-one optimization module designed to convert original quantum circuits into optimized versions that are more tailored for execution on classical computers.
\item [$C_2$] This paper presents the implementation and performance analysis of the all-in-cache simulation module with a high-speed simulation workflow.
\item[$C_3$] This paper conducts a comparative analysis of simulation performance utilizing qubit, gate, and circuit benchmarks on multi-GPUs against state-of-the-art simulators.
\end{description}

\subsection{Computational Artifacts}

% \artexpl{
% List the computational artifacts related to this paper along with their respective DOIs. Note that all computational artifacts may be archived under a single DOI.
% }

% \fixme{ fix the DOI at below.
% \artsampl{
% \begin{description}
% \item[$A_1$] https://doi.org/10.5281/zenodo.10889267
% \item[$A_2$] https://doi.org/10.5281/zenodo.10889267
% % \item[$A_2$] https://doi.org/ZZ.YYYY/zenodo.1XXXXX
% % \item[$A_3$] https://doi.org/ZZ.YYYY/zenodo.2XXXXX
% \end{description}
% }
% }

\textbf{For security purposes, to prevent unauthorized use, we kindly request that you contact the authors via email.}

%\artexpl{Provide a table with the relevant computational artifacts, highlight their relation to the contributions (from above) and point to the elements in the paper that are reproducible by each artifact, e.g., which figures or tables were generated with the artifact.}

% \artsampl{
% \begin{center}
% \begin{tabular}{rll}
% \toprule
% Artifact ID  &  Contributions &  Related \\
%              &  Supported     &  Paper Elements \\
% \midrule
% $A_1$   &  $C_1$ & Tables 1-2 \\
%         &        & Figure 3\\
% \midrule
% $A_2$   &  $C_2$ & Tables 2-3 \\
%         &        & Figures 1-2\\
% \midrule
% .. \\
% \bottomrule
% \end{tabular}
% \end{center}
% }

\begin{center}
\begin{tabular}{rll}
\toprule
Artifact ID  &  Contributions &  Related \\
             &  Supported     &  Paper Elements \\
\midrule
$A_1$ & $C_1$ & Figure 5 \\
\midrule
$A_2$ & $C_2$, $C_3$ & Figure 8 \\
& & Figure 9 \\
& & Figure 10 \\
& & Figure 11 \\
& & Figure 12 \\
%\midrule
\bottomrule
\end{tabular}
\end{center}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Artifact Identification}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \artexpl{
% Provide the following six subsections for each computational artifact $A_i$.
% }

\newartifact

\artrel

% \artexpl{
%     Briefly explain the relationship between the artifact and contributions.
% }

This artifact $A_1$ is an implementation of $C_1$, which is an optimization tool for doing the qubit reordering and gate fusion within the quantum circuits.

\artexp
%\artexpl{ Provide a higher level description of what outcome to expect from the corresponding experiments. Provide an explanation of how the results substantiate the main contributions.}

This artifact aims to transform any circuits (e.g., QFT, QAOA, or BV) into the optimized circuit file, which includes gate blocks, in-memory swapping (SQS), and cross-rank swapping (CSQS).
Specifically, the input format for the circuit is structured as follows.
\begin{center}
\begin{tcolorbox}[breakable]
\textbf{[Gate type] \textcolor{red}{[Target qubits]} [ID] [Remain info]}
\end{tcolorbox}
\end{center}

Given an example circuit represented in Figure 5 (a), along with our specified input format, the optimization module is capable of producing the optimized circuit as output.
\begin{center}
\begin{tcolorbox}[breakable]
\textbf{H \textcolor{red}{0} 0}
\\\textbf{ H \textcolor{red}{1} 1}
\\\textbf{ RZZ \textcolor{red}{2 4} 2}
\\\textbf{ RZZ \textcolor{red}{5 7} 3}
\\\textbf{ H \textcolor{red}{8} 4}
\\\textbf{ H \textcolor{red}{9} 5}
\\\textbf{ H \textcolor{red}{3} 6}
\\\textbf{ H \textcolor{red}{6} 7}
\\\textbf{ RZZ \textcolor{red}{0 2} 8}
\\\textbf{ RZZ \textcolor{red}{4 7} 9}
\\\textbf{ H \textcolor{red}{9} 10}
\\\textbf{ RZZ \textcolor{red}{1 8} 11}
\\\textbf{ RZZ \textcolor{red}{3 6} 12}
\\\textbf{ H \textcolor{red}{5} 13}
\end{tcolorbox}
\end{center}

The output resulting from the qubit reordering optimization should match Figure 5(b) as follows.
The target qubit for each original gate operation should not exceed the chunk size of 4, which is also marked in red.
\begin{center}
\begin{tcolorbox}[breakable]
\textbf{3} \textcolor{ForestGreen}{\# Gate Block Size}
\\\textbf{H \textcolor{red}{0} 0}
\\\textbf{H \textcolor{red}{1} 1}
\\\textbf{H \textcolor{red}{3} 6}
\\\textbf{1}
\\\textbf{SQS 3 0 1 3 4 5 7} \textcolor{ForestGreen}{\# In-memory swapping}
\\\textbf{4}
\\\textbf{RZZ \textcolor{red}{0 2} 2}
\\\textbf{RZZ \textcolor{red}{1 3} 3}
\\\textbf{RZZ \textcolor{red}{0 3} 9}
\\\textbf{H \textcolor{red}{1} 13}
\\\textbf{1}
\\\textbf{SQS 3 0 1 3 4 6 7}
\\\textbf{3}
\\\textbf{H \textcolor{red}{1} 7}
\\\textbf{RZZ \textcolor{red}{1 3} 12}
\\\textbf{RZZ \textcolor{red}{0 2} 8}
\\\textbf{1}
\\\textbf{SQS 2 0 2 6 7}
\\\textbf{1}
\\\textbf{CSQS 2 6 7 8 9} \textcolor{ForestGreen}{\# Cross-rank swapping}
\\\textbf{1}
\\\textbf{SQS 2 0 2 6 7}
\\\textbf{1}
\\\textbf{SQS 1 3 5}
\\\textbf{4}
\\\textbf{H \textcolor{red}{2} 5}
\\\textbf{H \textcolor{red}{2} 10}
\\\textbf{H \textcolor{red}{0} 4}
\\\textbf{RZZ \textcolor{red}{0 3} 11}
\end{tcolorbox}
\end{center}

After applying all features in this module, the result should match Figure 5(c). The diagonal gates, such as RZZ, within each gate block, will be merged without altering correctness.
To avoid excessive elaboration, detailed results are not provided.
Please verify this matter effortlessly through the scripts we provided.

To verify the optimized circuit executes in the correct sequence and with proper dependencies
on target qubits, one can utilize our validation script as follows.
\begin{center}
\begin{tcolorbox}[breakable,colback=blue!5!white,colframe=blue!75!black]
\textbf{\$ }\textcolor{ForestGreen}{\# switch workspace to the validatio directory}
\\
\textbf{\$ cd ./tests}
\\
\textbf{\$ }\textcolor{ForestGreen}{\# run the validation script}
\\
\textbf{\$ ./validate\_circuit\_order.sh}
\end{tcolorbox}
\end{center}


If all optimized circuits have the correct sequence, the message "Passed all circuit order validations" will be output to the terminal. Otherwise, a mismatch error will be invoked.

\arttime

% \artexpl{
% Estimate the time required to reproduce the artifact, providing separate estimates for the individual steps: Artifact Setup, Artifact Execution, and Artifact Analysis.
% }

The expected results of this module are listed as follows.
\begin{easylist}
& The required time for Artifact Setup is negligible if our provided raw circuit file is adopted. Otherwise, installing the Python package of the open-source project may take 5-10 minutes.
& For Artifact Execution, each optimized circuit of our benchmark is consistently generated within 0.5 seconds.
& For Artifact Analysis, the optimized circuit does not represent the actual simulation efficiency, so we refrain from discussing it for now.
\end{easylist}

\artin

\artinpart{Hardware}
% \artexpl{
% Specify the hardware requirements and dependencies (e.g., a specific interconnect or GPU type is required).
% }

No specific Hardware is required to execute the experiments.

\artinpart{Operating System}
We employ Docker with Ubuntu 22.04 and kernel version 5.15.0-1044-nvidia for our experiments. 
However, no specific operating system is required to execute the experiments.

\artinpart{Software}
% \artexpl{
% Introduce all required software packages, including the computational artifact. For each software package, specify the version and provide the URL.
% }

No specific software is required to execute the experiments.
However, for the convenience of downloading the open-source circuit generator and facilitating subsequent simulation stages, we still recommend installing all necessary environments at this stage.

\begin{easylist}
& In order to generate highly reproducible circuits in an open-source manner and facilitate direct comparisons with various works in one single execution environment, Python 3.10.12 should be used along with the following package dependencies. (i.e., using different configurations does not ensure running the experiments for all related works in one single environment):

    && attrs==20.3.0
    && cachetools==5.3.3
    && certifi==2021.5.30
    && charset-normalizer==3.3.2
    && cirq==0.13.1
    && cirq-aqt==0.13.1
    && cirq-core==0.13.1
    && cirq-google==0.13.1
    && cirq-ionq==0.13.1
    && cirq-pasqal==0.13.1
    && cirq-rigetti==0.13.1
    && cirq-web==0.13.1
    && contourpy==1.2.0
    && cuquantum-cu12==23.10.0
    && custatevec-cu12==1.5.0
    && cutensor-cu12==1.7.0
    && cutensornet-cu12==2.3.0
    && cycler==0.12.1
    && decorator==5.1.1
    && dill==0.3.8
    && duet==0.2.9
    && fonttools==4.49.0
    && google-api-core==1.34.1
    && google-auth==2.28.2
    && googleapis-common-protos==1.63.0
    && grpcio==1.62.1
    && grpcio-status==1.48.2
    && h11==0.9.0
    && httpcore==0.11.1
    && httpx==0.15.5
    && idna==2.10
    && iso8601==0.1.16
    && kiwisolver==1.4.5
    && lark==0.11.3
    && matplotlib==3.8.3
    && mpmath==1.3.0
    && msgpack==1.0.8
    && networkx==2.8.8
    && numpy==1.26.4
    && nvidia-cublas-cu12==12.3.4.1
    && nvidia-cuda-runtime-cu12==12.3.101
    && nvidia-cusolver-cu12==11.5.4.101
    && nvidia-cusparse-cu12==12.2.0.103
    && nvidia-nvjitlink-cu12==12.3.101
    && packaging==24.0
    && pandas==2.2.1
    && pbr==6.0.0
    && pillow==10.2.0
    && ply==3.11
    && protobuf==3.20.3
    && psutil==5.9.8
    && py==1.11.0
    && pyasn1==0.5.1
    && pyasn1-modules==0.3.0
    && pydantic==1.8.2
    && PyJWT==1.7.1
    && pyparsing==3.1.2
    && pyquil==3.0.1
    && python-dateutil==2.8.2
    && python-rapidjson==1.16
    && pytz==2024.1
    && pyzmq==25.1.2
    && qcs-api-client==0.8.0
    && qiskit==0.46.0
    && qiskit-aer-gpu==0.13.3
    && qiskit-terra==0.46.0
    && requests==2.31.0
    && retry==0.9.2
    && retrying==1.3.4
    && rfc3339==6.2
    && rfc3986==1.5.0
    && rpcq==3.11.0
    && rsa==4.9
    && ruamel.yaml==0.18.6
    && ruamel.yaml.clib==0.2.8
    && rustworkx==0.14.2
    && scipy==1.12.0
    && six==1.16.0
    && sniffio==1.2.0
    && sortedcontainers==2.4.0
    && stevedore==5.2.0
    && symengine==0.11.0
    && sympy==1.12
    && toml==0.10.2
    && tqdm==4.66.2
    && typing\_extensions==4.10.0
    && tzdata==2024.1
    && urllib3==2.2.1
\end{easylist}

\artinpart{Datasets / Inputs}

% \artexpl{
% Describe the datasets required by the artifact. Indicate whether the datasets can be generated, including instructions, or if they are available for download, providing the corresponding URL.
% }

To lessen the load on users for recompilation, the experimental inputs consist of a designated configuration file and a total of 17 distinct gates and circuits, accessible via the ./circuit directory.
% Alternatively, one can also generate all the required configuration files and circuits with the following command.
Alternatively, one can also generate all the raw circuits with the following command.

\begin{center}
\begin{tcolorbox}[breakable,colback=blue!5!white,colframe=blue!100!black]
\textbf{\$ }\textcolor{ForestGreen}{\# install required packages listed in the \emph{Software} section}
\\
\textbf{\$ pip3 install -r requirements.txt}
\\
\textbf{\$ }\textcolor{ForestGreen}{\# switch workspace to the following directory}
\\
\textbf{\$ cd ./optimizer}
\\
\textbf{\$ }\textcolor{ForestGreen}{\# generate raw circuits (e.g., BV, QAOA, ..., etc) }
\\
\textbf{\$ ./gen\_raw\_circuits.sh}
\\
\end{tcolorbox}
\end{center}


% \textbf{\$ make} \textcolor{ForestGreen}{\# build finder}
% \\
% \textbf{\$ ./gen\_all\_circuit\_files.sh}
%It's important to mention that the second command will download a file used for generating circuits from the public project located at https://github.com/qiboteam/qibojit-benchmarks.

\artinpart{Installation and Deployment}
% \artexpl{
% Detail the requirements for compiling, deploying, and executing the experiments, including necessary compilers and their versions.
% }
The version of the GNU g++ compiler used is 11.04.

% As in the previous section, the optimized inputs consist of the designated configuration files and a total of 17 distinct gates and circuits, accessible via the ./circuit directory.
% Alternatively, one can also generate all the configuration files and optimized circuits with the following command.
% \\
% \textcolor{ForestGreen}{\# switch workspace to the following directory}
% \\
% \textbf{\$ cd ./optimizer}
% \\
% \textcolor{ForestGreen}{\# complie}
% \\
% \textbf{\$ make -j}
% \\
% \textcolor{ForestGreen}{\# generate optimized circuits (e.g., BV, QAOA, QFT, ..., etc) }
% \\
% \textbf{\$ ./gen\_subcircuits.sh}

%The version of the GNU g++ compiler used is 11.04.

\artcomp

% \artexpl{
% Provide an abstract description of the experiment workflow of the artifact. It is important to identify the main tasks (processes) and how they depend on each other. 

% A workflow may consist of three tasks: $T_1, T_2$, and $T_3$. The task $T_1$ may generate a specific dataset. This dataset is then used as input by a computational task $T_2$, and the output of $T_2$ is processed by another task $T_3$, which produces the final results (e.g., plots, tables, etc.). State the individual tasks $T_i$ and provide their dependencies, e.g., $T_1 \rightarrow T_2 \rightarrow T_3$.

% Provide details on the experimental parameters. How and why were parameters set to a specific value (if relevant for the reproduction of an artifact), e.g., size of dataset, number of data points, input sizes, etc. Additionally, include details on statistical parameters, like the number of repetitions.
% }

A workflow may consist of two tasks: $T_1$ and $T_2$.
Task $T_1$ compiles the C++ source code for the all-in-one module.
Task $T_2$ leverages the module to transform the raw circuits in all experiments into optimized circuits.
The dependency of tasks is $T_1 \rightarrow T_2$
Note that the raw circuits have already been obtained in the \emph{dataset/input} section.

% A workflow may consist of two tasks: $T_1$ and $T_2$.
% Task $T_1$ is optional and involves downloading the circuit generator scripts from the open-source project located at https://github.com/qiboteam/qibojit-benchmarks.
% This step can be omitted since we have already organized the complete circuit in the ./circuit directory. 

% Task $T_2$ generates the optimized circuit from the original one.
% To fully demonstrate the impact of performance in the subsequent stages, 7 practical quantum circuits and 10 standard quantum gates are used as benchmarks.
% Of course, you may still generate specific simulation circuit files according to your needs, but please refer to the advanced user manual to complete this customized task.
%The dependencies for reproducing our work are as follows: $T_1 \rightarrow T_2$.

\artout
In terms of efficiency, the elapsed time for transforming any raw circuit is less than 1 second on a DGX-A100, thanks to the polynomial-time complexity of the implementation.

Moreover, this artifact demonstrates promising results in reducing the number of gate blocks.
For example, the 31-qubit QFT circuit with 496 gates is grouped into only 18 gate blocks.
Theoretically, memory access time could be reduced by a factor of 27 (496/18). However, in practice, this reduction is usually unattainable due to considerations involving compiler optimizations, making it more of a reference point.

The reductions in gate blocks result in fewer in-memory swaps and cross-rank swaps compared to other works, thereby enhancing an 8-fold times speedup while running the circuit through our simulation module ($A_2$) on the DGX-A100, a significance that is elaborated upon in more depth in the AE.

\newartifact

\artrel

This artifact $A_2$ is a comprehensive tool for quantum circuit simulation that orchestrates the complete implementation of $C_2$.
%Running this artifact with a performance profiler yields the results of $C_3$ on the given machines.
The integration of various benchmarks and other simulators can showcase the efficiency of $C_3$ (i.e., demonstrating higher efficiency compared to the other works).
Alongside the generated circuit via artifact $A_1$, this stage enables the presentation of a comprehensive performance report.
\artexp

The expected results of each benchmark on a DGX-A100 workstation are listed as follows.
These benchmarking results can dominate state vector-based simulation in various cases, as mentioned in 

\begin{easylist}
& QAOA Benchmark: \\Our work with fusion should get a performance improvement of 4.x compared to cuQuantum and aer with gate fusion, and our work in a single GPU without fusion still outperforms Aer and cuQuantum with fusion in 2 GPUs.
& QFT Benchmark: \\Our work with fusion should get a performance improvement of 4.x compared to cuQuantum and aer with gate fusion, and our work in a single GPU without fusion still outperforms Aer and cuQuantum with fusion in 2 GPUs.
& Qubit Benchmark: \\Our work should get an average performance improvement of 9.x compared to cuQuantum and Aer in various qubit scenarios.
& Strong Scaling Benchmark: \\This experiment demonstrates that our work has strong scaling capability, achieving an average performance improvement of 8.7x compared to cuQuantum and Aer in various rank scenarios.
& Gate Benchmark: \\ To show the versatility of various gates, our work should get an average performance improvement of 8.7x compared to cuQuantum and Aer.
& Circuit Benchmark: \\To show the versatility of various circuits, our work should get an average performance improvement of 9.x compared to cuQuantum and Aer.
& Breakdown of 34-qubit Simulation Time: \\Gate operation should occupy the most time. This experiment can be used to analyze the whole simulation process for different circuits.
& Breakdown of 34-qubit Simulation Time w/o NVLink and shared memory: \\The cross-rank swapping should occupy the most time. This experiment serves as a benchmark for comparison against NVLink and socket-based methodologies.
& Roofline Model of The 30-qubit H-gate Benchmark: \\Our work should be computation-bound, while QuEST should be memory-bound, highlighting the decisive difference that demonstrates us as the next-generation simulator.
\end{easylist}

\arttime

\begin{easylist}
& For Artifact Setup, the required time is negligible if our Dockerfile is adopted. 
Otherwise, installing the NVIDIA Driver, CUDA toolkit, and NCCL library may take up to 30 minutes, depending on network speed.

& For Artifact Execution, we provide the expected computational time of this artifact on a DGX-A100 as follows.
Notably, the proficiency with which information is gathered using a profiler varies depending on the familiarity with the operations.
    && QAOA Benchmark: 16 minutes
    && QFT Benchmark: 5 minutes
    && Qubit Benchmark: 4 minutes
    && Strong Scaling Benchmark: 3 minutes
    && Gate Benchmark: 15 minutes
    && Circuit Benchmark: 15 minutes
    && Breakdown of 34-qubit Simulation Time: 15 minutes
    && Breakdown of 34-qubit Simulation Time without NVLink: 150 minutes
    && Roofline Model: 3 minutes
& For Artifact Analysis, the required time is negligible when utilizing our provided script, which summarizes the results into a CSV and PDF file for each experiment.
%Otherwise, each experiment may take 5-10 minutes to discern the parameters and input for various simulators.
\end{easylist}

\artin

\artinpart{Hardware}

For the experiments, we use a DGX-A100 workstation comprising two AMD EPYC 7742 CPUs and eight NVIDIA A100 SXM GPUs interconnected via NVLink, boasting a bandwidth of 600GB/s.

\artinpart{Operating System}
We employ Docker with Ubuntu 22.04 and kernel version 5.15.0-1044-nvidia for our experiments. 
However, no specific operating system is required to execute the experiments.

\artinpart{Software}
We use NVCC ver. 12.3.107 and the NCCL library ver. 2.20.3.
To reproduce the related works, the Python environment matches that of artifact $A_1$. You also need cmake to build QuEST, the related work we compared our work against. The version of cmake we use is ver. 3.22.1.

\artinpart{Datasets / Inputs}
All circuit inputs can be obtained after completing the steps of artifact $A_1$.

\artinpart{Installation and Deployment}

For compilation, we use NVCC ver. 12.3.107 with the "-lnccl -arch=sm\_80 -O3 
-{}- jump-table-density=0 -maxrregcount=64" flags and the NCCL library ver. 2.20.3 for compiling the CUDA codes.

To compile the executable file, execute "make -j" in the terminal within the ./simulator directory of the workspace path, and no specific requirements for deploying our work.

To execute the experiments, ensure the configure and circuit files exist, then run it with the following suggested command.
\begin{center}
\begin{tcolorbox}[breakable,colback=blue!5!white,colframe=blue!100!black]
\textbf{\$ ./simulator/Quokka -i [configure file] -c [circuit file]}
\end{tcolorbox}
\end{center}

\artcomp

A workflow may consist of three tasks: $T_1$, and $T_2$.
The task $T_1$ generates specific configure files, quantum gates, and circuits as benchmarks with optimizations for the simulators\footnote{The task $T_1$ represents the entire process of artifact $A_1$. If already completed, please skip this step.
}.
These configurations and benchmarks are then used as input by computational task $T_2$.
The outputs can be directly displayed in the terminal.
The results can also be automatically summarized as a CSV and PDF file if one utilizes our provided scripts.
%With a comprehensive chart or additional plotting package in task $T_3$, exquisite performance reports can be presented.
The dependencies for reproducing our work are as follows: $T_1 \rightarrow T_2$.
The detailed step-by-step reproduction will be detailed in the Artifact Evaluation section.

The details of the experimental parameters are listed as follows.
\begin{easylist}
& In our simulator, specifying the size of the simulated qubits is achieved by switching the configuration file. This can be done by modifying the value of N in the .ini file.
& In our simulator, simulating different circuits only requires switching the .txt file without the need for recompilation.
Rest assured, our scripts, codes with comments, and README.md files offer abundant examples to aid in completing all experiments.
& The default number of qubits in the A100 scenario is set to 31 (this is the memory upper limit), but please adjust it according to your GPUs.
& There are 7 practical quantum circuits and 10 standard quantum gates used as benchmarks. 
You can still generate speciåfic simulation circuit files according to your needs, but please refer to the advanced user manual to complete this task.
& Given that the circuits executed in benchmarks and simulated scenarios are both large-scale, it is recommended to run the simulations multiple times to remove noise, even though running once is usually sufficient to indicate the simulation time.
\end{easylist}

\artout
Overall, we utilize the better elapsed time to identify a more effective simulation result.
A brief analysis and interpretation of each benchmark are listed below.
\begin{easylist}
& QAOA Benchmark:
\\This benchmark evaluates the overall simulation with gate fusion on a specific 31-qubit QAOA circuit.
Our work with gate fusion gets the fastest results on a DGX-A100.
& QFT Benchmark: 
\\This benchmark evaluates the overall simulation with gate fusion on a specific 31-qubit QFT circuit.
Our work with gate fusion gets the fastest results on a DGX-A100.
& Qubit Benchmark:
\\This benchmark evaluates the time per gate for the standard Hadamard gate with qubits ranging from 24 to 31.
It demonstrates the performance of the simulator under varying memory consumption levels.
Our work gets the fastest results for all cases on an A100.
& Strong scaling Benchmark:
\\This benchmark evaluates the time per gate for the standard Hadamard gate with ranks ranging from 1 to 8 exponentially.
It demonstrates the robust scalability of the simulator under varying GPU ranks.
Our work gets the fastest results for all cases on a DGX-A100.
& Gate benchmark:
\\This benchmark evaluates the time per gate for different types of gates on a 31-qubit system.
It demonstrates the high performance of each implementation for all varying gates.
Our work gets the fastest results for all cases on an A100.
& Circuit benchmark:
\\This benchmark evaluates the time per gate for different types of practical circuits on a 31-qubit system.
It demonstrates the high performance of each implementation for varying circuits.
Our work gets the fastest results for all cases on an A100.
& Breakdown of 34-qubit simulation time:
\\This hotspot analysis demonstrates the elapsed times of different techniques, providing insight into the performance bottlenecks of different models, with NVLink serving as the transfer medium for cross-rank communication.
Observing the changes in elapsed time, it can be noted that introducing in-memory swapping and cross-rank swapping is highly beneficial.
& Breakdown of 34-qubit simulation time without NVLink and shared memory:
\\This hotspot analysis demonstrates the elapsed times of different techniques, providing insight into the performance bottlenecks of different models without relying on NVLink for cross-rank communication. Observing the changes in elapsed time, it can be noted that utilizing NVLink for cross-rank swapping is highly beneficial.
& Roofline model of the 30-qubit H-gate benchmark: \
\\This analysis is typically used to determine whether the application is computation-bound or memory-bound.
By utilizing the Nsight Compute profiler, it is evident that our simulator is computation-bound across different levels of GPU.
For other simulators (we take QuEST as an example), the performance is significantly limited by memory bandwidth.
\end{easylist}

% \newartifact

% \artexpl{
% Provide the same type of information as done for Computational Artifact $A_1$.
% }


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  AE Appendix
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newpage
\appendixAE

\arteval{1}
\artin

% \artexpl{
% Provide instructions for installing and compiling libraries and code. 
% Offer guidelines on deploying the code to resources.
% }
To lessen the load on users for recompilation, the experimental inputs consist of a designated configuration file and a total of 17 distinct gates and circuits accessible via the ./circuit directory. 
Alternatively, one can also generate all the raw circuits with the following command
\begin{center}
\begin{tcolorbox}[breakable,colback=blue!5!white,colframe=blue!100!black]
\textbf{\$ }\textcolor{ForestGreen}{\# install required packages listed in the \emph{Software} section}
\\
\textbf{\$ pip3 install -r requirements.txt}
\\
\textbf{\$ }\textcolor{ForestGreen}{\# switch workspace to the following directory}
\\
\textbf{\$ cd ./optimizer}
\\
\textbf{\$ }\textcolor{ForestGreen}{\# download qasm.py from another github project.}
\\
\textbf{\$ }\textcolor{ForestGreen}{\# generate raw circuits (e.g., BV, QAOA, ..., etc) }
\\
\textbf{\$ ./gen\_raw\_circuits.sh}
\\
\textbf{\$ }\textcolor{ForestGreen}{\# compile the optimization module }
\\
\textbf{\$ make -j}
\end{tcolorbox}
\end{center}

\artcomp
Please switch the workspace to the optimizer directory and call the script to generate the gate blocks for the raw gate and circuit files.
% \artexpl{
% Describe the experiment workflow. 
% If encapsulated within a workflow description or equivalent (such as a makefile or script), clearly outline the primary tasks and their interdependencies. Detail the main steps in the workflow. Merely instructing to “Run script.sh” is inadequate.
% }
\begin{center}
\begin{tcolorbox}[breakable,colback=blue!5!white,colframe=blue!100!black]
\textbf{\$ }\textcolor{ForestGreen}{\# switch workspace to the following directory}
\\
\textbf{\$ cd ./optimizer}
\\
\textbf{\$ }\textcolor{ForestGreen}{\# execution the optimization module for all raw circuits}
\\
\textbf{\$ ./gen\_gateblocks.sh }
\end{tcolorbox}
\end{center}

The compilation of the optimization module only requires using g++ to compile the finder.cpp file. The `gen\_gateblocks.sh' bash script iteratively optimizes and formalizes the raw circuits into the optimized circuits for our simulator via the gate block finding algorithm. The gates and circuits benchmark includes: ['bv', 'hs', 'qaoa', 'qft', 'qv', 'sc', 'vc', 'h', 'u', 'x', 'cx', 'cp', 'swap', 'rx', 'ry', 'rz', 'rzz'].



\artout

% \artexpl{
% \begin{itemize}
%     \item Provide a description of the expected results and a methodology for evaluating these results. 
%     \item Explain how the expected results from the experiment workflow correlate with the contributions stated in the article. 
%     \item For example, if the article presents results in a figure, the artifact evaluation should also produce a similar figure, depicting the same generalizable outcome. Authors must focus on these aspects to reduce the time required for others to understand and verify an artifact.
% \end{itemize}
% }

This artifact generates the necessary configuration and optimized circuit for the $A_2$ simulation module.
Although a comprehensive understanding of the optimization requires quantum computing expertise, we provide a simplified explanation.
Given the raw circuit with a specific chunk size, the target qubit of the output should fit within this region by inserting in-memory swapping and cross-rank swapping operations. 
This ensures that subsequent simulations can fully leverage the cache properties for quantum gate simulation.

The format for the circuit file should be as follows.
For detailed information, please refer to the provided README.md file.
\begin{center}
\begin{tcolorbox}[breakable]
\textbf{[Gate type] \textcolor{red}{[Target qubits]} [ID] [Remain info]}
\end{tcolorbox}
\end{center}

Using Figure 5(a) as an example, the raw circuit file is as follows.
\begin{center}
\begin{tcolorbox}[breakable]
\textbf{H \textcolor{red}{0} 0}
\\\textbf{ H \textcolor{red}{1} 1}
\\\textbf{ RZZ \textcolor{red}{2 4} 2}
\\\textbf{ RZZ \textcolor{red}{5 7} 3}
\\\textbf{ H \textcolor{red}{8} 4}
\\\textbf{ H \textcolor{red}{9} 5}
\\\textbf{ H \textcolor{red}{3} 6}
\\\textbf{ H \textcolor{red}{6} 7}
\\\textbf{ RZZ \textcolor{red}{0 2} 8}
\\\textbf{ RZZ \textcolor{red}{4 7} 9}
\\\textbf{ H \textcolor{red}{9} 10}
\\\textbf{ RZZ \textcolor{red}{1 8} 11}
\\\textbf{ RZZ \textcolor{red}{3 6} 12}
\\\textbf{ H \textcolor{red}{5} 13}
\end{tcolorbox}
\end{center}

Next, we need to understand how to apply our tool to create the correct format for our simulation module.
\begin{center}
\begin{tcolorbox}[breakable,colback=blue!5!white,colframe=blue!100!black]
\textbf{\$ ./optimizer/finder [target file] [cache size] [rank size] [qubit size] [apply in-memory swapping] [apply cross-rank swapping] [fusion size] [apply fusion technique]}
\end{tcolorbox}
\end{center}


\begin{easylist}
& The function of each parameter is listed as follows.
%&& [optimizer]: The execution file.
&& [target file]: The raw circuit file. 
&& [cache size]: The $2^{cache \ size}$ can not exceed the shared memory size of the GPU rank.
&& [rank size]: The $2^{rank \ size}$ can not exceed the primary memory size of the GPU rank.
&& [apply in-memory swapping]: Enable the in-memory swapping.
&& [apply cross-rank swapping]: Enable cross-rank swapping for multiple GPU environments.
&& [fusion size]: The $2^{fusion \ size}$ represents the region for gate fusion; this size should always not be larger than the cache size.
&& [apply fusion technique]: Enable gate fusion.
\end{easylist}

Now, input the following command to generate the optimized circuit as Figure5 (b).
\begin{center}
\begin{tcolorbox}[breakable,colback=blue!5!white,colframe=blue!100!black]
\textbf{\$ ./optimizer/finder ./circuit/example/raw.txt 4 8 10 1 1 0 0}
\end{tcolorbox}
\end{center}

The output should be as follows.
\begin{center}
\begin{tcolorbox}[breakable]
\textbf{3} \textcolor{ForestGreen}{\# Gate Block Size}
\\\textbf{H \textcolor{red}{0} 0}
\\\textbf{H \textcolor{red}{1} 1}
\\\textbf{H \textcolor{red}{3} 6}
\\\textbf{1}
\\\textbf{SQS 3 0 1 3 4 5 7} \textcolor{ForestGreen}{\# In-memory swapping}
\\\textbf{4}
\\\textbf{RZZ \textcolor{red}{0 2} 2}
\\\textbf{RZZ \textcolor{red}{1 3} 3}
\\\textbf{RZZ \textcolor{red}{0 3} 9}
\\\textbf{H \textcolor{red}{1} 13}
\\\textbf{1}
\\\textbf{SQS 3 0 1 3 4 6 7}
\\\textbf{3}
\\\textbf{H \textcolor{red}{1} 7}
\\\textbf{RZZ \textcolor{red}{1 3} 12}
\\\textbf{RZZ \textcolor{red}{0 2} 8}
\\\textbf{1}
\\\textbf{SQS 2 0 2 6 7}
\\\textbf{1}
\\\textbf{CSQS 2 6 7 8 9} \textcolor{ForestGreen}{\# Cross-rank swapping}
\\\textbf{1}
\\\textbf{SQS 2 0 2 6 7}
\\\textbf{1}
\\\textbf{SQS 1 3 5}
\\\textbf{4}
\\\textbf{H \textcolor{red}{2} 5}
\\\textbf{H \textcolor{red}{2} 10}
\\\textbf{H \textcolor{red}{0} 4}
\\\textbf{RZZ \textcolor{red}{0 3} 11}
\end{tcolorbox}
\end{center}

For the output, observe that the target qubit for each original gate operation should not exceed the chunk size of 4, as marked in red. Now, we continue by enabling the diagonal fusion function.
Please input the following command to generate the circuit files with all functions in this module.
\begin{center}
\begin{tcolorbox}[breakable,colback=blue!5!white,colframe=blue!100!black]
\textbf{\$ ./optimizer/finder ./circuit/example/raw.txt 4 8 10 1 1 4 1}
\end{tcolorbox}
\end{center}

The output should be as follows.
\begin{center}
\begin{tcolorbox}[breakable]
\textbf{3}
\\\textbf{H \textcolor{red}{0} 0}
\\\textbf{H \textcolor{red}{1} 1}
\\\textbf{H \textcolor{red}{3} 6}
\\\textbf{1}
\\\textbf{SQS 3 0 1 3 4 5 7}
\\\textbf{2}
\\\textbf{D4 \textcolor{red}{0 1 2 3} 0.75390225434330471 \emph{...}}
\\\textbf{H \textcolor{red}{1} 13}
\\\textbf{1}
\\\textbf{SQS 3 0 1 3 4 6 7}
\\\textbf{2}
\\\textbf{H \textcolor{red}{1} 7}
\\\textbf{D4 \textcolor{red}{0 1 2 3} -0.83907152907645244 \emph{...}}
\\\textbf{1}
\\\textbf{SQS 2 0 2 6 7}
\\\textbf{1}
\\\textbf{CSQS 2 6 7 8 9}
\\\textbf{1}
\\\textbf{SQS 2 0 2 6 7}
\\\textbf{1}
\\\textbf{SQS 1 3 5}
\\\textbf{4}
\\\textbf{H \textcolor{red}{0} 4}
\\\textbf{RZZ \textcolor{red}{0 3} 11}
\\\textbf{H \textcolor{red}{2} 5}
\\\textbf{H \textcolor{red}{2} 10}
\end{tcolorbox}
\end{center}

This resulting output should match Figure 5(c).
As mentioned above, you can also observe that the target qubit for each original gate operation should not exceed the chunk size of 4, as marked in red.
Moreover, the RZZ gates with IDs 2, 3, and 9 are now merged into a single D4 gate, and RZZ gates with IDs 7, 8, and 12 are also merged into a single D4 gate.
The symbol "\emph{...}" represents the remaining information of the fused gates.

Congratulations! You now have enough knowledge to discern the correctness of more complex circuits in our benchmark.
Of course, we also invite you to verify via our scripts.

\textbf{[Auto-validation]}
To validate that the optimized circuit executes in the correct sequence and with proper dependencies on target qubits, one can utilize our validation script. The processes are outlined as follows:
\begin{center}
\begin{tcolorbox}[breakable,colback=blue!5!white,colframe=blue!100!black]
\textbf{\$ }\textcolor{ForestGreen}{\# switch workspace to the validation directory}
\\
\textbf{\$ cd ./tests}
\\
\textbf{\$ }\textcolor{ForestGreen}{\# run the validation script}
\\
\textbf{\$ ./validate\_circuit\_order.sh}
\end{tcolorbox}
\end{center}

This script will invoke `dump\_order.py' for both the original circuit and the optimized one to perform detailed checking.
In summary, `dump\_order.py' traverses the circuit's operations on qubits and restores the optimized circuit to its original positions according to the sequence of swaps performed during optimization.
After the `diff' command in the script is used to compare the differences between the two circuits, the validation results will be provided.

If all pairs of circuits are identical, it indicates that the transformed circuit is correct.
In this case, the message "Passed all circuit order validations" will be output to the terminal.
Otherwise, the mismatch error will be invoked.

\arteval{2}

\artin

If you are using the Docker environment provided by us, you can skip this step.
Otherwise, please install NVCC version 12.3.107, NCCL library version 2.20.3, cmake 3.22.1 and the Python packages for the related works on your machine.
Nsight System v2023.2.3 is required to analyze the execution time. Other versions contain unexpected bugs from NVIDIA and may not work successfully.

\begin{easylist}
& To install the NVCC toolkit, please follow the instructions on the official website: \\ https://docs.nvidia.com/cuda/cuda-installation-guide-linux/index.html

& To install the NCCL library, please follow the instructions on GitHub: https://github.com/NVIDIA/nccl

& To install Nsight System v2023.2.3, please download and follow the instructions on the official website: https://developer.nvidia.com/gameworksdownload

& To install the Python 3.10.12 package for the related works, please follow the instructions as follows.
\begin{center}
\begin{tcolorbox}[breakable,colback=blue!5!white,colframe=blue!100!black]
\textbf{\$ }\textcolor{ForestGreen}{\# install required packages listed in \emph{Software} section}
\\
\textbf{\$ pip3 install -r requirements.txt}
\\
\textbf{\$ }\textcolor{ForestGreen}{\# switch workspace to the following directory}
\\
\textbf{\$ cd ./simulatior}
\\
\textbf{\$ }\textcolor{ForestGreen}{\# compile the simulation module }
\\
\textbf{\$ make -j}
\end{tcolorbox}
\end{center}
\end{easylist}

\artcomp

To run each benchmark, we now need to understand how to apply our tool to create
the correct format for our simulation module.
\begin{center}
\begin{tcolorbox}[breakable,colback=blue!5!white,colframe=blue!100!black]
\textbf{\$ ./simulator/Quokka -i [configure file] -c [circuit file]}
\end{tcolorbox}
\end{center}

\begin{easylist}
& The function of each parameter is listed as follows.
%&& [simulator]: The execution file.
&& [configure file]: The configure file for the simulations.
&& [circuit file]: The circuit file for the simulations.
\end{easylist}

The example of the circuit file is the output of the optimizer, as mentioned above, and the example of the configure file with comments to explain each parameter is provided below.
\begin{center}
\begin{tcolorbox}
\textbf{[system]}
\\
\textbf{total\_qbit=31} \textcolor{ForestGreen}{// Total qubit for simulation}
\\
\textbf{rank\_qbit=0} \textcolor{ForestGreen}{ // The total ranks for running the simulation.}
\\
\textbf{buffer\_qbit=28} \textcolor{ForestGreen}{// The size of buffer for data transfer.}
\end{tcolorbox}
\end{center}

The example for running the specific circuit and configuration file is as follows:
\begin{center}
\begin{tcolorbox}[breakable,colback=blue!5!white,colframe=blue!100!black]
\textbf{\$ ./simulator/Quokka -i ./circuit/sub0/30/gpu.ini -c ./circuit/sub0/30/h30.txt}
\end{tcolorbox}
\end{center}

For the initial step, please switch the workspace to the `benchmarks' directory, and then build QuEST, the related work that we compared our work against.

\begin{center}
  \begin{tcolorbox}[breakable,colback=blue!5!white,colframe=blue!100!black]
\textbf{\$ }\textcolor{ForestGreen}{\# switch workspace to the following directory}
\\
\textbf{\$ cd ./bechmarks}
\\
\textbf{\$ }\textcolor{ForestGreen}{\# build QuEST simulator for benchmarks}
\\
\textbf{\$ ./build\_QuEST.sh}
  \end{tcolorbox}
\end{center}

The executable of QuEST will be built and located in `./benchmarks/QuEST/build/demo' relative to the artifact's root directory.

Then, to run the experiments and generate the figures automatically, as illustrated in the paper, please keep your working directory in `./benchmarks' and run the commands listed below.

\begin{easylist}    
  & QAOA Benchmark:
  \begin{center}
  \begin{tcolorbox}[breakable,colback=blue!5!white,colframe=blue!100!black]
  \textbf{\$ ./1a\_strong\_scale\_qaoa.sh $>$ qaoa.csv}
  \\
  \textbf{\$ python3 1\_strong\_scale\_circuit.py qaoa.csv qaoa.pdf}
  \end{tcolorbox}
  \end{center}
  && The first command will execute the QAOA simulation in our simulator, Aer simulation, and cuQuantum, while redirecting the results to the CSV file. The second command can generate a PDF file, as shown in Figure 8(a) in our paper.
  & QFT Benchmark: 
  \begin{center}
  \begin{tcolorbox}[breakable,colback=blue!5!white,colframe=blue!100!black]
  \textbf{\$ ./1b\_strong\_scale\_qft.sh $>$ qft.csv}
  \\
  \textbf{\$ python3 1\_strong\_scale\_circuit.py qft.csv qft.pdf}
  \end{tcolorbox}
  \end{center}
  && Similarly to the QAOA benchmark, the first command will execute the QFT simulation in all simulators while redirecting the results to the CSV file. The second command can generate a PDF file, as shown in Figure 8(b) in our paper.
  & Qubit Benchmark:
  \begin{center}
  \begin{tcolorbox}[breakable,colback=blue!5!white,colframe=blue!100!black]
  \textbf{\$ ./2a\_qubit\_benchmark.sh $>$ qubit.csv}
  \\
  \textbf{\$ python3 2a\_qubit\_benchmark.py qubit.csv qubit.pdf}
  \end{tcolorbox}
  \end{center}
  && The first command will execute the 31-qubit h-gate simulation in all simulators ranging from 24 to 30 qubits while redirecting the results to the CSV file. The second command can generate a PDF file, as shown in Figure 9(a) in our paper.
  & Strong scaling Benchmark:
  \begin{center}
  \begin{tcolorbox}[breakable,colback=blue!5!white,colframe=blue!100!black]
  \textbf{\$ ./2b\_strong\_scale.sh $>$ scaling.csv}
  \\
  \textbf{\$ python3 2b\_strong\_scale.py scaling.csv scaling.pdf}
  \end{tcolorbox}
  \end{center}
  && The first command will execute the strong scaling test for 31-qubit h-gate in all simulators while redirecting the results to the CSV file. The second command can generate a PDF file, as shown in Figure 9(b) in our paper.
  & Gate benchmark:
  \begin{center}
  \begin{tcolorbox}[breakable,colback=blue!5!white,colframe=blue!100!black]
  \textbf{\$ ./3a\_gate\_benchmark.sh $>$ gates.csv}
  \\
  \textbf{\$ python3 3a\_gate\_benchmark.py gates.csv gates.pdf}
  \end{tcolorbox}
  \end{center}
  && The first command will execute the strong scaling test for 31-qubit simulation of various types of gates in all simulators while redirecting the results to the CSV file. The second command can generate a PDF file, as shown in Figure 10(a) in our paper.
  & Circuit benchmark:
  \begin{center}
  \begin{tcolorbox}[breakable,colback=blue!5!white,colframe=blue!100!black]
  \textbf{\$ ./3b\_circuit\_benchmark.sh $>$ circuits.csv}
  \\
  \textbf{\$ python3 3b\_circuit\_benchmark.py circuits.csv circuits.pdf}
  \end{tcolorbox}
  \end{center}
  && The first command will execute the strong scaling test for 31-qubit simulation of various types of circuits in all simulators while redirecting the results to the CSV file. The second command can generate a PDF file, as shown in Figure 10(b) in our paper.
  & Breakdown of 34-qubit simulation time:
  \begin{center}
  \begin{tcolorbox}[breakable,colback=blue!5!white,colframe=blue!100!black]
  \textbf{\$ ./4a\_breakdown.sh $>$ nvlink.csv}
  \\
  \textbf{\$ python3 4a\_breakdown.py nvlink.csv nvlink.pdf}
  \end{tcolorbox}
  \end{center}
  && The first command will execute nsys profiler for all 34-qubit simulations of various types of circuits in all simulators while redirecting the results to the CSV file. The second command can generate a PDF file, as shown in Figure 11(a) in our paper.
  & Breakdown of 34-qubit simulation time without NVLink and shared memory:
  \begin{center}
  \begin{tcolorbox}[breakable,colback=blue!5!white,colframe=blue!100!black]
  \textbf{\$ ./4b\_breakdown.sh $>$ socket.csv}
  \\
  \textbf{\$ python3 4b\_breakdown.py socket.csv socket.pdf}
  \end{tcolorbox}
  \end{center}
  && The first command will execute nsys profiler for all 34-qubit simulations of various types of circuits in all simulators without applying NVLink and shared memory while redirecting the results to the CSV file. The second command can generate a PDF file, as shown in Figure 11(b) in our paper.
  \\To disable NVLink and shared memory support, the script includes specific parameters for the nccl library, such as `NCCL\_P2P\_DISABLE=1 and NCCL\_SHM\_DISABLE=1'.
  & Roofline model:
  \begin{center}
  \begin{tcolorbox}[breakable,colback=blue!5!white,colframe=blue!100!black]
  \textbf{\$ ./5\_roofline.sh $>$ roofline.csv}
  \\
  \textbf{\$ python3 5\_roofline.py roofline.csv roofline.pdf}
  \end{tcolorbox}
  \end{center}
  && The first command will execute the NSight compute profiler for all 30-qubit h-gate simulations in all simulators while redirecting the results to the CSV file. The second command can generate a PDF file, as shown in Figure 12 in our paper.
  \\ In general, this script only generates result for a single rank. To include additional ranks, such as RTX 4090 and 3090, please adhere to our guidelines and manually input their specifications into the script.
\end{easylist}

\artout
The figures and tables in our experimental results can be automatically produced by our script in the previous subsection, and the analysis for each experiment is listed below.
\begin{easylist}
  & QAOA and QFT Benchmark:
  \\ The strong scaling test for these two typical benchmarks comprehensively demonstrates our achievements in surpassing other simulators across various metrics. From one to eight GPUs, with or without diagonal fusion enabled, all our experiments have consistently outperformed other simulators with an average speedup of 8x times.
  & Qubit Benchmark and Strong Scaling Benchmark:
  \\ This experiment serves to support a more detailed comparison. We utilize the standard 31-qubit H-gate at this stage and validate its effects across different qubits and under strong scaling tests. These results indicate that our simulator achieves the best 9x acceleration and demonstrates excellent scalability.
  & Gate benchmark and Circuit benchmark:
  This experiment aims to demonstrate that our implementation techniques can be applied across various scenarios, such as standard gates and circuits. Among them, cuQuantum exhibits the poorest simulation performance, while we boast the best execution efficiency. The fundamental reason lies in our specific optimizations for each gate rather than relying solely on transpilation techniques in IBM-qiskit preprocessing. On DGX-A100, our related improvement in efficiency (i.e., time per gate) ranges between 5-10x.
  & Breakdown of 34-qubit simulation time with and without NVLink:
  \\ We profile our simulation at this stage using the NVIDIA nsys profiler. The results from the profiler should be divided by the total number of machines, as the measured data represents the total time of all machines. The elapsed time for AIO optimization is measured separately, but since it typically consumes less than 0.1\% of the time, it is not merged into the profiler to reduce the programming overhead. Primarily, despite the introduction of numerous swap operations, the majority of the time is dedicated to gate operations. 
  Additionally, when NVLink and shared memory on the host are disabled, there is a notable increase in data transfer time.
  This observation indicates that socket-based approaches may not be entirely optimal for supercomputing environments. Therefore, the approaches that offer high bandwidth and low latency are necessary, exemplified by the latest NVLink technology.
  & Roofline model:
  \\ In order to fairly compare the optimized results, all reports of the roofline model are obtained by the Nsight Compute profiler without additional manual processing. The result clearly shows that our simulator is computation-bound, and the other is the memory-bound program.
  We have overwhelmingly superior performance in both TFLOPS (8x) and Arithmetic Intensity (96x) on DGX-A100.
   We also demonstrate this performance profiling on RTX-3090 and RTX-4090. 
   The results indicate that our performance in FLOPS on RTX-3090 surpasses that of QuEST on A100.
\end{easylist}

\subsection{Summary}
\textbf{Queen}: ``My little princesses and princes, the other self-proclaimed state-of-the-art works are either irreproducible or indeed quite slow. 
Until when should this truth be concealed?
I'm so bored. Would you play with me?"

==> contents/aio_optimization_module.tex <==
\section{All-in-one Optimization Module}
\label{sec:aio_optization_module}

\begin{figure*}[tb!]
\centerline{\includegraphics[width=1.98\columnwidth]{figures/swapExample.pdf}}
\caption{The circuit diagrams of various optimized techniques for Queen.}
\label{fig:swapExam}
\end{figure*}

% 在實際運行模擬之前, 部分的模擬器整合了數個優化電路的部件，並安插在模擬器的不同階段中。
% 最為知名的優化技術為 gate fusion 與 qubit reordering.
% gate fusion 通常是將電路進行 transpile 成當前環境所能運行的 gate, 並提供 gate 合併的方式來減少計算.
% qubit reordering 則是透過 swapping qubit 的技法來減少跨機器的溝通時間.
%Prior to simulation execution, specific simulators incorporate optimized circuit components like gate fusion and qubit reordering, embedding them at different stages.
%Gate fusion typically transpiles quantum circuits into executable gates for the given environment while merging multiple gates to reduce computations.
%Qubit reordering utilizes swapping techniques to decrease communication time across distributed machines.

% 這些優化缺乏完整的流程指引, 使得使用者無從了解其對於能真正影響效率
% 這也是研究者鮮少甚至難以探討的原因之一。
% 有鑑於此，一套適用於所有優化的前處理模組的開發勢在必行
%Given these challenges, the development of a preprocessing module applicable to all optimizations is imperative.
% All-in-one Optimization Module 不僅能統一所以優化於同一階段，其更能在相對於運算時間 的 1% 以內完成，並帶來超過 2 倍的優化.
%Prior to simulation execution, specific simulators incorporate optimized circuit components, including gate fusion and qubit reordering, embedding them at different stages to enhance simulation efficiency
%However, these optimizations lack comprehensive workflow guidelines, posing challenges for users in understanding the actual efficiency impact and hindering further developments.
%To address these challenges, the proposed all-in-one optimization module unifies all optimizations at the same stage and completes within 1\% of computation time, leading to more than a twofold improvement.

% 既存的量子電路優化技法，在 high level 層面都能被歸納為同一種技法。
% 其為：在限制條件下, 使用一個集合將 gate 搜集在一起, 其中限制條件可以明示成 gate 所需要的 target gubit 小於 chunk size）
% 因此，我們將這樣的集合定義為 gate block (GB) 並表示如下.
% 其中, 最小的限制就是 dependency 與 涉及到的 qubit 總數
% 如此，我們定義一個 集合, called gate block (GB) 來搜集特定 gate as Equation~\ref{eq:gb}.

From a broad perspective, the existing quantum circuit optimization techniques, such as gate fusion and qubit reordering, can be generalized into a unified mathematical optimization problem with minor adjustments to constraints.
That is, these methods seek to minimize a specific cost function within a given circuit.
For instance, the cost objective is to minimize the count of fused gates and the frequency of data transfers for gate fusion and qubit reordering, respectively.
% Developing an algorithm to solve multiple problems perfectly aligns with the core design principle of ``\emph{Less is More}" in Queen.

To formalize this process, we define a set, denoted as gate block (\textit{GB}), to aggregate these specific gates.
The constraints typically entail dependencies ($\textit{dep}$) and the total number of involved target qubits (\textit{chunkSize}), as shown in Equation~\ref{eq:gb}.

\begin{equation}
\begin{array}{ll}
\label{eq:gb}
%GB = \{ g_i \in gateList \ | \ \underset{i \in \mathbb{N}}{\bigcup} dep(g_i) \leq \mathit{C} \}
\textit{GB} = \{ g \in \textit{gateList} \}, \ \| \underset{g \in \textit{GB}}{\bigcup} \textit{dep}(g) \| \leq \textit{chunkSize}
\end{array}
\end{equation}

Then, as illustrated in Equation~\ref{eq:gbs}, all determined gate blocks are included in a more extensive set \textit{GBs}. where the intersection of any two gate blocks is an empty set, and the union of all gate blocks is equivalent to \textit{gateList}.


\begin{equation}
\begin{array}{ll}
\label{eq:gbs}
% \underset{GBs}{\text{argmax}} \sum\limits_{GB \in GBs} \text{max} \|GB\|
%\underset{GBs}{\text{argmax}}  \|GB\|, GB \in GBs
% GBs = \{ GB_i \ | \ i \in \mathbb{N} \},
% \bigcup_{GB_i \in GBs} GB_i = \text{gateList}, \\
% GB_i \cap GB_j = \emptyset, \text{ if } i \leq j 
\textit{GBs} = \{ \textit{GB}_i \} , \ \textit{GB}_i \cap \textit{GB}_j = \varnothing, \forall i<j  \\ 
\end{array}
\end{equation}

% By doing so，這些優化問題得以寫成 最小化 GBs 的數量 
% 這種 最小化問題難以被實作完成，故我們將其改寫成等價的最大化問題，其目標為最大化在GBs 的 平均GB 大小 as Equation~\ref{eq:min}.
By applying the definitions provided above, the optimization problems can be efficiently re-formulated by minimizing the number of \textit{GBs}. 
To facilitate the implementation of the optimization process programmatically, we transform it as an equivalent maximization problem, seeking to maximize the average size of \textit{GB} within \textit{GBs}, as depicted in Equation~\ref{eq:min}.

\begin{equation}
\begin{array}{lll}
\label{eq:min}
%\underset{GBs}{argmin} & \|GBs\|  \\ 
\underset{\textit{GBs}}{\text{argmin}} \ \|\textit{GBs}\| \iff \underset{\textit{GBs}}{\text{argmax}} \ \sum\limits_{\textit{GB} \in \textit{GBs}} \frac{  \|\textit{GB}\| } { \|\textit{GBs}\| } \\
% \underset{GBs}{argmax} & \ AVG(GB_i) \\
% s.t. & GBs = \{ GB_i \}_i , GB_i \cap GB_j = \emptyset, \forall i<j  \} 
\end{array}
\end{equation}

% 根據功能的不同，剩餘的部分用來做細微的處理.
% After 完成，GBs 做為答案被回傳於 Line 15.
The pseudo-code presented in Algorithm~\ref{algo:find_gb} exhibits how the finding process fits the maximization problem within polynomial time.
During each iteration (in Line 4), the algorithm updates dependencies in Line 6 and determines the maximum \textit{GB} in Line 7.
Specific functionality for different problems is dealt with in Lines 8-13.
Following the completion of the algorithm, the optimized list \textit{GBs} is returned in Line 15.

\begin{algorithm}[hbt!]
  \caption{Pseudo-code to find the gate blocks.}
  \label{algo:find_gb}
  \SetKwInOut{kwInput}{Input}
  \SetKwInOut{kwOutput}{Output}
  \SetKwProg{Fn}{Function}{:}{end}
  \SetKw{Continue}{continue}

  \Fn
    {findGBs({\textit{gateList}, $\mathit{N}$, \textit{chunkSize}, isFusion}) } {
      chunkSet $\gets$ $\{q_{0}, \dots, q_{\textit{chunkSize}-1}\}$

      \textit{GBs}.append(setupGB(\textit{gateList}, chunkSet))

      \While{\textit{gateList} $\neq$ None} {
        prevSet $\gets$ chunkSet

        updateDependency(\textit{gateList}, $\mathit{N}$)

        chunkSet $\gets$ findMaxGate(\textit{gateList}, \textit{chunkSize})

        \If {isFusion} {
            doFusion(\textit{GBs}, $\mathit{N}$, \textit{chunkSize}, chunkSet)

            \Continue
        }

        insertQubitSwaps(\textit{GBs}, prevSet, chunkSet)

        \textit{GBs}.append(setupGB(\textit{gateList}, chunkSet))

      }

      \Return \textit{GBs}
    }

\end{algorithm}

Algorithm~\ref{algo:aio_opt} outlines the pseudo-code for the complete all-in-one optimization, utilizing $\mathit{R}$, $\mathit{C}$, $\mathit{F}$ to denote the relationship of memory size, cache size, and the scope of gate fusion, respectively.
This optimization consists of three-level progress, each employing the \textit{findGBs}() function with decreasing order, sequentially occurring in Lines 1, 4, and 8.
With each progression, the search scope becomes more refined, ultimately leading to an optimization duration that ordinarily occupies less than 1\% of the total simulation time.

% Figure~\ref{fig:swapExam} shows a random circuit with 14 gates by applying different optimization techniques.
% 圖中每個圖示 with its ID number 表是一個指定的 gate, 其座落的位置表示所設計到的 target qubit.
% 在一班的模擬器中, The simulation for the un-optimized circuit % 涉及到了許多的 10 個 記憶體等級的存取, 4 個 跨機器等級的存取.
% 在具有 cache 級的模擬器, 這樣的 cirucit 還是只 萃出 4個 cache 等級的運算於記憶體等級的存取, 這樣是沒有完整利用cache 的特性
In~\figurename{~\ref{fig:swapExam}}(a), there is a raw circuit made up of fourteen quantum gates.
Each symbol in the circuit corresponds to a different gate with a unique ID number, and the position of the symbol represents the targeted qubit.
Simulating this raw circuit with the previous simulators requires ten memory-level accesses and four cross-rank-level accesses. 
Even with cache-level optimization, the circuit only engages four cache-level accesses, indicating an inefficient exploitation of cache characteristics.

\figurename{~\ref{fig:swapExam}} (b) demonstrates the optimized circuit resulting from qubit reordering by our proposed swapping operations (denoted by crosses).
All quantum gates in the circuit can be accommodated within the cache region, requiring five memory-level accesses and only one cross-rank-level access for swapping operation.
Furthermore, upon enabling all optimization features, as shown in~\figurename{~\ref{fig:swapExam}} (c), gates can be seamlessly fused within the cache region with optimal circuit depth.
%In Fig. 5, we explain our strategy with 8 threads.
% We demonstrate the entire process with an example corresponding to the algorithm steps in~\figurename{~\ref{fig:finder_process}}. In summary, our
This AIO module can guarantee that computations predominantly maximize the cache utilization while minimizing the number of gate operations with high scalability.

% Figure~\ref{fig:swapExam}(b) 展示了 qubit reordering 的結果.
% 再經過 swapping 的技法後 (圖中的叉叉), all gates are 座落於 cache size 的區域中.
% 這樣的電路, 3 次的 memory-level accesses and 1 次的 cross-rank-level accesses.
% 在開啟所有的優化功能後, as Figure~\ref{fig:swapExam}(c), gate 得以在 cache 區間被融合. 
% 引入這樣的技法, 電路能確保運算盡可能在 cache 且做最少的運算


\begin{algorithm}[hbt!]
  \caption{Pseudo-code of all-in-one optimization.}
  \label{algo:aio_opt}
  \SetKwInOut{kwInput}{Input}
  \SetKwInOut{kwOutput}{Output}

  \kwInput{\textit{gateList}, $\mathit{N}$, $\mathit{R}$, $\mathit{C}$, $\mathit{F}$, \textit{isFusion}}
  \kwOutput{\textit{GB}}

\textit{devGBs} $\gets$ \textit{findGBs}(\textit{gateList}, $\mathit{N}$, $\mathit{N}$-$\mathit{R}$, 0)\tcp*{1-level}

  \For(\tcp*[f]{2-level}){devGB $\in$ devGBs} {
    \textit{gateList} $\gets$ setupList(\textit{devGB})

    \textit{GB} $\gets$ \textit{findGBs}(\textit{gateList}, $\mathit{N}$, $\mathit{C}$, 0) 

    \If {isFusion} {
      \For(\tcp*[f]{3-level}){GB $\in$ GBs} {
        \textit{gateList} $\gets$ setupList(\textit{GB})

        \textit{fusedGBs} $\gets$ \textit{findGBs}(\textit{gateList}, $\mathit{N}$, $\mathit{F}$, 1) 
      }
      \textit{GBs} $\gets$ \textit{fusedGBs}
    }
  }

  \SetKwFunction{SFA} {}
  \SetKwProg{Fn}{Function}{:}{end}
  \SetKw{Continue}{continue}

  %\Fn
  %  {finder({gateList, N, chunkSize, isFusion}) } {
  %    chunkSet $\gets$ $\{q_{0}, \dots, q_{chunkSize-1}\}$

      %SGBs.append(setupSGB(gateList, chunkSet))

      %\While{gateList $\neq$ None} {
       % prevSet $\gets$ chunkSet

        %updateDependency(gateList, N)

        %chunkSet $\gets$ findMaxGate(gateList, chunkSize)

        %\If {isFusion} {
        %    doFusion(SGBs, N, chunkSize, chunkSet)

        %    \Continue
        %}

        %insertQubitSwaps(SGBs, prevSet, chunkSet)

        %SGBs.append(setupSGB(gateList, chunkSet))

      %}

      %\Return SGBs
    %}
\end{algorithm}

==> contents/cross_device.tex <==
\subsection{Cross-rank Swapping (XRS)}
\label{sec:xdev_swapping}
Cross-rank swapping (XRS) constitutes the communication technique for applying the swapped qubit to a local rank.
Compared to IMS, XRS is commonly used to swap all required qubits for reducing the data movement across multiple hardware devices and machines~\cite{cache_blocking, cpu_gpu_communication, mpiQulacs, cuQuantum}.

As depicted in \figurename{~\ref{fig:nccl}}(a), the standard implementation is accomplished through the repetition of three phases, including gathering, cross-rank transfer, and scattering.
This approach necessitates that endpoints manage potentially fragmented data transfer with two supplementary buffers, and current implementations cannot guarantee the swap of all qubits in a single operation.
Consequently, this not only significantly degrades overall operational efficacy but also forces redundant buffers to consume the already scarce memory resources.

Fortunately, these challenges are effectively alleviated with the adoption of our innovative design.
First, the AIO optimization ensures that data sent to a peer is concentrated.
Then, the XRS facilitates an all-to-all communication pattern, allowing for the swapping of all qubits once and for all.
As a result, this coordinated approach maximizes data transfer throughput and minimizes redundant buffer usage.

Algorithm~\ref{algo:xrs} illustrates the comprehensive process of the XRS swap within CUDA-based implementations to align with our practical codes\footnote{
To achieve optimal communication performance for the NVIDIA environment with NVLink, similar to the latest cuQuantum and Aer simulators, we choose to leverage the NVIDIA Collective Communication Library (NCCL)~\cite{nccl}. For portability across CPUs and AMD GPUs, the API in NCCL can be seamlessly replaced with MPI and RCCL libraries, offering comparable communication performance, respectively.
}.
The entire transfer process comprises iteratively performing NCCL all-to-all operations in Lines 2-11, succeeded by memory copy operations in Lines 14.
Upon reaching the buffer of other ranks, the data are copied back to the memory to ensure that subsequent instructions can smoothly utilize the advantages of shared memory for subsequent gate operations, as mentioned in Section~\ref{sec:gate_operations}.

% https://jdhao.github.io/2019/09/21/latex_algorithm_pseudo_code/
\begin{algorithm}
\caption{Pseudo-code of cross-rank swapping}
\label{algo:xrs}
    \SetKwInOut{KwIn}{Input}
    \SetKwInOut{KwOut}{Output}
    \KwIn{The number of swap pairs ($S$) and the receive buffer size ($2^B$).}
    
    \For{$\textit{offset} \gets 0 $ to $2^{N-R-S}$ by $2^{B-S}$}{
        \tcp{1. cross-rank transfer}
        \For{$grp \gets 0$ to $2^{R-S}-1$ }{
            \tcc{Each NCCL operation is enclosed in a pair of the \emph{ncclGroup} primitives to transfer data bidirectionally.}
            ncclGroupStart() \\
            \For{$rSend \gets 0$ to $2^{S}-1$} { 
                \For{$rRecv \gets 0$ to $2^{S}-1$} {
                    ncclSend() \\
                    ncclRecv()
                }
            }
            ncclGroupEnd() \\
        }
        \tcp{2. copy}
        \For{$grp \gets 0$ to $2^{R-S}-1$} {
            \For{$r \gets 0$ to $2^{S}-1$} {
                memcpyRecvBufToSv()
            }
        }
    }
\end{algorithm}


\begin{figure}[tb!]
\centerline{\includegraphics[width=.95\columnwidth]{figures/nccl.pdf}}
\caption{Data communication for cross-rank swapping.}
\label{fig:nccl}
\end{figure}

In \figurename{~\ref{fig:nccl}}(b), we present an illustrative example demonstrating the transfer between two ranks. 
Obviously, our new technique condenses the three-step transfer into two steps and minimizes the buffer requirement by half, compared to the original method. 
Furthermore, the AIO optimization guarantees that the required swapped qubits are tightly continuous, thereby thoroughly optimizing bidirectional bandwidth.

Note that it is crucial to consider network congestion for high-speed data transfers.
Our XRS implementation utilizes all-to-all collective communications to exchange state vectors among machines and devices.
This communication pattern is symmetric, and there should not be any hotspots.
Therefore, the proposed approach achieves full hardware bandwidth utilization while keeping high scalability and portability.

==> contents/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

% Performance
%  1. 我們是最快
%  2. 從 Memory-Bound 到 Compute-Bound.
%
% Scalibility
%  1. 跨節點效能估算
%  2. Weak Scaling 特性
%
% Portability (已經說明了)
%  我們的 Concept 是 General 可以很快速移值到 AMD GPU

To address the considerations of the diverse users across various experimental platforms, we conduct the discussion to delve into the critical aspects and the further improvement of Queen, particularly emphasizing performance and scalability.

%\subsection{Performance}
\emph{\textbf{Performance.}}
As illustrated in \figurename{~\ref{fig:roofline_model}}, the roofline model not only demonstrates the absolute dominance of Queen in performance but also highlights the specific limitations of prior SOTA simulators.
It is evident that the workload of traditional QCS is memory-bound and restricted by the GPU memory bandwidth.
Through our cache-friendly simulation scheme, we effectively eliminate this critical bottleneck, transforming QCS into a compute-bound application.

Moreover, Queen can be significantly accelerated with enhanced computing power. For instance, leveraging a next-generation GPU such as the GB200, which offers 90 TFLOPS compared to 9.7 TFLOPS for the A100, we expect a 9x speedup of the simulation.
Such substantial improvements are unattainable with conventional memory-bound simulators~\cite{QuEST, Aer_sim, cuQuantum, Cirq} in high-performance computing.

It is worth noting that Queen has not yet reached the roof.
This is primarily due to the model being computed with ideal FMA intrinsics managed by SM units in Nsight Compute.
The practical QCS involves numerous memory operations to compute the effect of each quantum gate and the instruction mix of the workload currently limits further improvements.
Therefore, it is crucial that we need to redesign a new accelerator for Queen to achieve its maximum capability.

%Our simulator, as depicted in the roofline model in \figurename{~\ref{fig:roofline_model}}, does not reach the roof. This is due to the instruction mix of the workload. Nevertheless, we achieve a remarkable speedup of up to 10x, which is attributable to the significant increase in arithmetic intensity and the efficiency of our cache-friendly algorithms.

%On average, our simulator can achieve a speedup of 9x over other state-of-the-art (SoTA) simulators, including QuEST, Qiskit-Aer, and cuQuantum. The workload of quantum circuit simulation (QCS) is traditionally memory-bound. However, with our cache-friendly algorithms for QCS, it shifts to being compute-bound.

%Our simulator, as depicted in the roofline model in \figurename{~\ref{fig:roofline_model}}, does not reach the roof. This is due to the instruction mix of the workload. Nevertheless, we achieve a remarkable speedup of up to 10x, which is attributable to the significant increase in arithmetic intensity and the efficiency of our cache-friendly algorithms.

% It is worth noting that our simulator can be further accelerated with increased computing power. For instance, utilizing a next-generation GPU such as the GB200, which offers 90 TFLOPS compared to 9.7 TFLOPS for the A100, we expect a 9x speedup of the simulation. This substantial improvement would not be achievable with conventional memory-bound simulators~\cite{QuEST, Aer_sim, cuQuantum, Cirq} in the high-performance computing domain.

%\subsection{Scalability}
\emph{\textbf{Scalability.}}
While the DGX-A100 workstation serves as our primary experimental environment, our XRS is not limited to multiple devices but also encompasses multiple machines and nodes.
We have extended the NCCL support to include the GPU-RDMA transfer technique that spans across ranks for QCS.
As a result, we term it cross-rank swapping (XRS).

Since the performance of data transfer for $2^\mathit{N}$ memory space is consistent, we can conduct the analysis to provide the correct direction for further research.
In general, the bidirectional bandwidth of NVLink between any two GPUs in the DGX-A100 is 600 GB/s.
Suppose we connect multiple machines with InfiniBand fabric, and each machine has 8x 200 Gbps InfiniBand NICs; then the inter-GPU communication bandwidth across machines would be 200 Gbps on average, which is \((200 \times 2) \div (600 \times 8) = 1/12\) of NVLink.
This result was replicated successfully in a similar network configuration.

Subsequently, our XRS accounts for only 10\% of simulation time on average in the circuit benchmarks.
Therefore, the total execution time would increase to 2.1 times (\(10\% \times 12 + 90\% \times 1 \)), meaning our MPI version with GPU-RDMA would run at 47.6\% of the speed over InfiniBand compared to NVLink.
%Still, our Queen outperforms all previous multi-rank GPU-based simulators~\cite{cpu_gpu_communication, cache_blocking, cuQuantum}.

%Despite potential concerns regarding portability when utilizing NVLink, it is recommended to employ these fastest communication techniques to meet high-performance demands.
Despite potential concerns regarding portability when utilizing NVLink, we recommend temporarily employing these fastest transfer techniques to meet high-performance demands.
With this in mind, NVIDIA GB200 NVL72~\cite{gh200_nvl72}, featuring 5th generation NVLink with bandwidth capabilities of 130 TB/s, emerges as a promising scalable solution for GPU-based QCS.

%In general, the bidirectional bandwidth of NVLink between any two GPUs in the DGX-A100 is 600 GB/s.
%Suppose we connect multiple machines with InfiniBand fabric, and each machine has 8x 200 Gbps InfiniBand NICs; then the inter-GPU communication bandwidth across machines would be 200 Gbps on average, which is \((200 \times 2) \div (600 \times 8) = 1/12\) of NVLink.
%As illustrated in \figurename{~\ref{fig:ana_all}}, XRS accounts for about 10\% of simulation time on average.
%Thus, the total execution time would increase to \(10\% \times 12 + 90\% = 2.1\) times, meaning our MPI version would run at 47.6\% of the speed over InfiniBand compared to NVLink.


%Although we only evaluated performance on a single node with multiple GPUs, our approach is general and applicable to multi-node environments, and we have also implemented an MPI version.

% Thanks to our AIO optimization module, in most cases, the number of cross-rank swaps (XRS) and the workload on a node remain constant with an increasing number of nodes and qubits, demonstrating the weak scaling property.

%To reduce the overhead of communication when simulating across multiple nodes, it is important to use the remote direct memory access (RDMA) technique for QCS~\cite{rdma_sim}.
%In general, the bidirectional bandwidth of NVLink between any two GPUs in the DGX-A100 is 600 GB/s.
%Suppose we connect multiple machines with InfiniBand fabric, and each machine has 8x 200 Gbps InfiniBand NICs; then the inter-GPU communication bandwidth across machines would be 200 Gbps on average, which is \((200 \times 2) \div (600 \times 8) = 1/12\) of NVLink.
%As illustrated in \figurename{~\ref{fig:ana_all}}, XRS accounts for about 10\% of simulation time on average.
%Thus, the total execution time would increase to \(10\% \times 12 + 90\% = 2.1\) times, meaning our MPI version would run at 47.6\% of the speed over InfiniBand compared to NVLink.

% In supercomputing environments, it is advisable to utilize the fastest communication techniques.
% With this in mind, NVIDIA GB200 NVL72~\cite{gh200_nvl72}, featuring 5th generation NVLink technology with bandwidth capabilities of 130 TB/s, emerges as a promising solution for QCS in a supercomputing environment.


% \subsection{Portability}
% As the key concept in the proposed methodology centers around the effective usage of caches and the reduction of interprocessor communications, our approach is general, scalable, and highly portable.
% Thus, our code can be quickly ported to AMD GPUs, as AMD offers ROCm and RCCL, which resemble CUDA and NCCL, respectively.


==> contents/postscript.tex <==
\section{Postscript}
\label{sec:postscript}
My name is Chuan-Chi Wang, a Ph.D. student at National Taiwan University.
This project was completed with the help of several awesome classmates, and we all share the same dream of performance optimization. I will not forget you all.

If you are passionate about performance optimization in quantum circuit simulation, I am truly happy to connect with you through this paper\footnote{This paper was written within less than a day by myself, so there may be some mistakes or typos that need correction. However, the performance results provided are all reproducible. For further details or questions, please feel free to email me, and I will respond privately.
}.
Nevertheless, the recent wave of malicious comments and ridicule has left me mentally and physically exhausted.
Maybe working on optimizations without the proper background naturally leads to such outcomes.

When I was young, I was taught that if I can not measure up, I should admit my shortcomings and humbly seek guidance.
But recently, the attitude of some top conferences has been quite disappointing to me.
Forgive me, my dear truth. I can not play games with such creepy gangsters.
Maybe I am not suited for academic research.

Of course, I will continue to uphold my pursuit of truth.
However, due to the comments from these masters, I will likely be shifting to another field soon.
My friends, if you found my papers helpful, feel free to say hi if we meet in the future.
Well, it is time for you to take QueenV3 to the next level.
Love you all.


==> contents/ralated_work.tex <==
\section{Related Work}
\label{sec:related_work}
Quantum circuit simulation can be typically categorized into state vector-based and tensor network-based approaches.
While tensor networks are limited in terms of interpretability and scalability, state vector-based QCS is widely preferred for its superior ability to represent complex quantum circuits with high scalability and parallelization accurately.
%Additionally, state vector-based QCS is highly parallelizable, making it ideal for execution on high-performance computer architecture.
%~\cite{QuEST, 45qubit, Aer_sim, cuQuantum, Cirq}.
To achieve effective and scalable QCS, it is essential to integrate complementary optimization techniques, including \emph{optimizing data locality}, \emph{increasing scalability}, and \emph{decreasing gate operations}.

\emph{\textbf{Optimizing Data Locality.}}
In state vector-based QCS, simulating $\mathit{N}$ qubits requires a memory capacity of $2^\mathit{N}$, leading to extensive memory access during operations directly.
In scenarios involving multiple machines or devices, it causes significant data transfers across the network.
The cross-rank swaps~\cite{cuQuantum, mpiQulacs} are proposed to alleviate this issue, while some studies~\cite{cache_blocking, cpu_gpu_communication} focus on optimising circuits to reduce the total number of data movements.
These approaches do not consider the dependencies between quantum gates, posing a significant risk of rapid degradation in larger clusters.
The hybrid approach presented in HyQuas~\cite{HyQuas} allows for switching between gate operations in the cache and fused gate operations via external libraries during the simulation process.
However, these two techniques represent orthogonal concepts.

Our proposed AIO module fully accounts for these dependencies and quantum gates, resulting in significant improvements in data transfer at the cache level and can be employed to address simulations in large clusters directly.
When integrated with our AIC module, our solution effectively resolves performance bottlenecks and can be readily adapted to diverse computing architectures without the limitations on other hardware-specific computing libraries.
%that have plagued QCS for over a decade.

\emph{\textbf{Increasing Scalability.}}
For the purpose of enhancing scalability, several simulators support multiple GPUs~\cite{cuQuantum, Aer_sim, Cirq} and distributed machines~\cite{QuEST, 45qubit} using communication libraries like NCCL and MPI.
Quokka~\cite{NTU_SSD} and SnuQS~\cite{park2022snuqs} utilize SSDs to extend the memory capacity cost-effectively and efficiently.
Nevertheless, the former only supports CPU-based simulation, whereas the latter relies heavily on a RAID-0 system with io\_uring.
Q-GPU~\cite{Q-GPU} systematically expands the available device memory for GPUs from host memory by leveraging the codes of the IBM-Aer simulator.
Pessimistically, with substantial updates to the IBM-Aer simulator, this work requires involvement from subsequent contributors.

In the current phase, these simulators are unable to perform the all-in-cache simulation. Hence, we plan to incorporate and enhance various functionalities in the future comprehensively.

\emph{\textbf{Decreasing Gate Operations.}}
This technique, commonly referred to as gate fusion, is employed to merge multiple gates into a single generic gate~\cite{45qubit, qHiPSTER, HyQuas, Aer_sim}.
Although reducing the total number of gates can potentially decrease memory access due to the memory-bound property, these fused gates typically are less efficient and may require additional performance evaluation.
%For instance, fusing an excessive number of CNOT gates in Quantum Fourier Transform (QFT) with distinct target qubits can lead to fused gates with too many qubits and exponentially growing unitary complexity.
In such cases, a cost function is typically employed to determine the necessity of merging between gates.
Among numerous fusion techniques, diagonal optimization is a proven technique that can simultaneously reduce the number of gates while maintaining efficiency for high-performance computing~\cite{qaoa_arxiv, juliQAOA}.

%both the simulation and circuit analysis levels.
% \emph{\textbf{Maximizing Parallelism.}}
% A multitude of studies have focused on applying parallelization to enhance the simulation performance across both homogeneous and heterogeneous systems.
% Within CPU architectures, multithreading and AVX vectorization techniques are implemented to exploit computational resources fully~\cite{qHiPSTER}.
% In GPUs, renowned for their extensive thread capabilities, maximizing parallelism strategies leads to superior performance against homogeneous systems~\cite{QuEST, Aer_sim, cuQuantum}.
% These techniques can be extended to encompass multi-rank scenarios for further performance improvement~\cite{QuEST, mpiQulacs, cpu_gpu_communication}.

==> contents/simulation_module.tex <==
\section{All-in-Cache Simulation Module}
\label{sec:simulation_module}
\begin{comment}
%Our quantum simulation is implemented with CUDA and runs on NVIDIA GPU. In this section, we will discuss how we implemented general gates, in-memory swapping, and cross-rank swapping.
In this section, we elaborate on three fundamental simulation methodologies within our simulation workflow: quantum gate operations, in-memory swapping, and cross-rank swapping.
In our pursuit of optimal performance, these implementations are tailored for CUDA on NVIDIA GPUs, integrating a comprehensive range of hardware and software techniques.

%Our proposed simulation can % 分類成 all-in-cache simulation.
% 徹底地解決了所有模擬器所遇到的效能的瓶頸
% the algorithm 展示了 simulation 的 flow.
% 其中, qubit的優化會被整理在
Our proposed simulation belongs to the category of all-in-cache simulation, effectively solving the performance issues faced by existing simulators. The pseudo-code of the simulation workflow is presented in Algorithm~\ref{algo:simulation_flow}. The algorithm establishes a high-performance simulation approach by replacing redundant memory accesses and cross-rank accesses with swap techniques in Lines 3 and 5. 
When it comes to gate operations, the simulator executes them in the cache sequentially in a block-by-block manner in Lines 7-10.
\end{comment}

% In this section, we elaborate the AIC simulation by representing the pseudo-code. Later, we discuss about the detail of the operations in AIC.

% The pseudo-code of the all-in-cache (AIC) simulation workflow is presented in Algorithm~\ref{algo:simulation_flow}. The algorithm establishes a high-performance simulation approach by replacing redundant memory accesses and cross-rank accesses with swap techniques in Lines 3 and 5. 
% When it comes to gate operations, the simulator executes them in the cache sequentially in a block-by-block manner in Lines 7-10.

The pseudo-code for the AIC simulation process is presented in Algorithm~\ref{algo:simulation_flow}.
This simulation takes an optimized circuit as the input and iterates through the gate blocks, as indicated in Line 1.
When encountering different types of gate blocks, the simulation performs cross-rank swaps (Line 3), in-memory swaps (Line 5), and in-cache operations with the block-by-block scheme (Lines 7-11).
In the pursuit of optimal performance on NVIDIA multi-GPUs, all implementations are tailored for CUDA, integrating a comprehensive range of hardware and software techniques in the subsequent subsection.

%. In this section, we will discuss how we implemented general gates, in-memory swapping, and cross-rank swapping.
%The pseudo-code for the AIC simulation workflow is outlined in Algorithm~\ref{algo:simulation_flow}. This simulation takes an optimized circuit as the input and iterates through the gate blocks, as indicated in Line 1. Depending on the type of gate block encountered, the simulation performs cross-rank swaps (Line 3), in-memory swaps (Line 5), and block-by-block operations (Lines 7-11). The gate blocks belonging to the former two swap operations may contain multiple pairs of exchanged qubits. To efficiently execute these swaps in a single operation, we will elaborate on the implementation details in the following subsections.

%Similarly, optimizing the performance of block-by-block gate operations requires code optimization. Detailed implementation strategies will be provided in the subsequent subsection.

\begin{algorithm}[hbt!]
  \caption{Pseudo-code of all-in-cache simulation.}
  \label{algo:simulation_flow}
  \SetKwInOut{kwInput}{Input}
  \SetKwInOut{kwOutput}{Output}
  \kwInput{The initialized stateVector and gateBlocks}
  \kwOutput{The simulated amplitude in stateVector}
  \For(\tcp*[f]{Scan gate block}){\textnormal{gateBlock $\in$ gateBlocks}} {
    \uIf {\textnormal{isCrossRankSwap(gateBlock)}} {
        stateVector$\gets$doCrossRankSwap(stateVector)
    }
    \uElseIf {\textnormal{isInMemSwap(gateBlock)}} {
        stateVector $\gets$ doInMemSwap(stateVector)
    }
    \Else (\tcp*[f]{Do quantum gate operations in cache}){
        \For {\textnormal{chunk $\in$ stateVector}} {
            \For {\textnormal{gate $\in$ gateBlock}} { 
                chunk $\gets$ doOperation(gate, chunk)
            }
        }
    }
  }  
\end{algorithm}

% In the forthcoming sections, we explore detailed implementation specifics and uncover techniques aimed at enhancing the speed of the three primary operations within our AIC simulation module.

\subsection{In-cache Gate Operations in Block-by-block Scheme}
\label{sec:gate_operations}
% 在整個 quantum computing 中, Quantum Gate Operations 是最基礎的執行單元, 其可以構築一個 quanutm circuit 並被進一步地 apply 到 實際應用中
% 以最有效率地方式實作 gate 行為, 表示著可以模擬器更快速地完成任務
In general, quantum gates are the foundational unit of computational operations in quantum computing and shape the landscape of quantum algorithms.
Within these algorithms, a quantum circuit is formed by applying diverse types of quantum gate operations to tackle practical challenges in the specific application domains.
The optimization of gate operations can lead to heightened efficiency, enabling simulations to complete complex tasks in less time.
%In essence, the expediting of gate operations can significantly facilitate the development of quantum algorithms.

% Compared to the past simulators,
% 在過去實作的 simulation 中, gate Operations 會被視為矩陣的模式來做運算, 並一個 gate-by-gate 的模式來模擬。
% 然而, 這樣粗糙的技法完全沒有徹底運用模擬裝置的運算特性, 並讓進階技法不能加以實施
% 為此，我們的模擬器提出加速優化的關鍵瓶頸，針對其給予應硬的解法
In previous quantum circuit simulators, gate operations are computed using matrix multiplications and simulated in a gate-by-gate scheme.
However, those legacy approaches fail to utilize the computational mechanisms of classical computers fully, thereby impeding the adoption of advanced high-performance techniques.
To rectify the situation, our simulator introduces a series of strategies to expedite simulation and eliminate performance bottlenecks, delineated as follows.
%The strategies are delineated as follows.

\emph{\textbf{Increase data locality.}}
% 將 state vector 分成數個不重疊的 chunk, 在不違反輸出的正確性之下 以chunk-by-chunk 的方式模擬最有效地提高能資料的重複使用性.
% 其中, 須將 chunk size 明確地 mapping 到 cache 空間, 如此才能確保 運算不會涉及到 記憶體等級的存取, 已達到最好的快取利用率.
% 此外, 我們將資料 主動地放入 shared memory 來保證 GPU cahce 能有效地被 directly programable 地掌控
% 如此，更能對 thread block 怎麼被分配到 streaming multiprocessor 的系列操作做最佳化
To enhance data reuse, the state vector is partitioned into non-overlapping chunks, where each GPU thread block exclusively processes states within its designated chunk.
Gates are grouped into gate blocks through our AIO optimization module, which guarantees that all operations within a block can be applied to a chunk without requiring data exchange beyond the chunk boundaries.
The simulation follows the determined gate block sequentially, resulting in a substantial improvement in data locality compared to alternative simulators.
Moreover, we actively place data into shared memory to explicitly control the use of the on-chip GPU memory.
This approach enables improved management of GPU performance tuning and thread block allocation to stream multiprocessors, leading to enhanced overall performance.

\begin{comment}
%To enhance data reuse, the state vector is partitioned into several non-overlapping chunks and executed sequentially in a chunk-by-chunk manner.
%To optimize data reuse, the state vector is divided into distinct, non-overlapping chunks, with each GPU thread block exclusively handling states within a designated chunk. 
%Gates are also grouped into several gate blocks by our AIO optimization module. Our AIO optimization module ensures that gates in a gate block can be applied to a chunk without the need for data exchange beyond the chunk boundaries. The simulation is performed in a block-by-block manner. By doing so, we achieve significant improved data locality compared to other simulators.
%Our AIO optimization module plays an important role to group gates into as few gate blocks as possible to reduce the global memory accesses.
To enhance data reuse, the state vector is partitioned into non-overlapping chunks, where each GPU thread block exclusively processes states within its designated chunk.
Gates are grouped into gate blocks through our AIO optimization module, which guarantees that gates within a block can be applied to a chunk without requiring data exchange beyond the chunk boundaries.
The simulation follows a block-by-block approach, resulting in a substantial improvement in data locality compared to alternative simulators.
Our AIO optimization module plays a crucial role in minimizing global memory accesses by efficiently grouping gates into as few gate blocks as possible.
% The simulation flow should follow a specific gate order under the guidance of our AIO optimization module to ensure output correctness.
% It is also necessary to map the chunk size into the cache space to prevent additional memory-level accesses and maximize cache utilization.
It is also necessary to adjust the chunk size correctly according to the size of the GPU cache to prevent additional memory-level accesses and maximize cache utilization.
% Moreover, actively placing data into shared memory allows for explicit control of the GPU cache through programming behavior.
Moreover, actively placing data into shared memory allows us to explicitly control the use of the GPU cache to improve performance further.
This approach enables improved management of GPU performance tuning and thread block allocation to stream multiprocessors (SMs), leading to enhanced overall performance.
\end{comment}


\emph{\textbf{Decrease stall barriers.}} % loop unrolling, lower sync operation
% 在 開源的 GPU 專案的實作中, 每個 threads 被安排去 accessing 一個 single quantum state, 
% 這樣的運算模式在 GPU 的架構中非常沒有效率 
% 以模擬層面來說, 根據涉及到不同 target qubit 數量運算時, 部分的 thread 被迫不去做運算以保持資料正確性.
% 以實際執行層面來說, 在 NVIDIA 的機器中, thread 是以 warp 的方式同時做運算, 這樣的運算不能使 warp 中的 thread 需要額外的暫停 與 同步的 overhead
% 實務上, 我們讓每個 thread 能去管裡多個 state, 在引入 loop unrolling 的技法後, warp 中的 thread 得以最低的 stall barrier 方式執行.
%In the implementation of most open-source GPU simulators, individual threads are assigned to access a single quantum state, a computational approach that proves highly inefficient for modern GPU architectures.
%In the implementation of most open-source GPU simulators, each thread handles a single quantum state. However, this approach has drawbacks.
%In the context of quantum simulation, when operations involve different numbers of target qubits, some threads are forced to abstain from computation to maintain data integrity, especially when applying a gate with control qubits.
%When operations in a gate block involve different numbers of target qubits and control qubits, tasks cannot be distributed evenly. Some threads need to wait on the barrier without any computation to maintain data integrity.
% In terms of hardware execution of NVIDIA ranks, the 32 threads within a warp execute simultaneously, resulting in additional stall barriers and synchronization overhead. (這句話怪怪的)
%To address these performance challenges, we unroll the loops, which means that each thread manages multiple states. Loops are unrolled per gate, which means that each gate could have different loop unrolling factors. This approach ensures that threads always have evenly distributed tasks to perform before encountering a barrier, effectively minimizing the time spent on barriers.
In open-source GPU simulators~\cite{QuEST, cpu_gpu_communication, mpiQulacs}, each thread typically manages a single quantum state in its implementation.
However, this approach can lead to uneven task distribution when operations involve varying numbers of target and control qubits. 
As a result, most threads in a thread block must wait at barriers without performing any computations to preserve data integrity, which negatively impacts performance.
To overcome this challenge, we adopt loop unrolling, allowing each thread to handle multiple states to utilize computational resources fully.
This technique is applied to each gate individually, ensuring the optimal unrolling factors for minimizing thread management and loop overhead without unnecessary stall barriers.

%This strategy effectively enables the threads in warps to continue running without unnecessary stall at barriers.
%the threads in warps can continue running without unnecessary stalls at barriers, which greatly enhances performance
%This strategy allows tasks to be distributed evenly among threads, minimizing the time spent at barriers and enhancing overall efficiency.
%This strategy % 有效地減少 time spent at barriers, 使得每個 thread in warps 能在不被暫停的情況下持續運行, 

\begin{comment}
\emph{\textbf{Optimize utilization of GPU resources.}}
% texture memory
% 類似與 rendering 圖象的應用, Quantum Circuit Simulation 中存在著複數個 gate type, such as diagonal and unitary gate, 這些 是能用 texture memory 來減少 memory 存取次數與提高 bandwidth.
% 類似與 rendering 圖象的應用, Quantum Circuit Simulation 中存在著複數個有參數的 gate type, 像是 diagonal and unitary gate。 這些參數屬於常數，能使用專為常數設計的 texture memory 來減少 memory 存取次數與提高 bandwidth.
% 這使得部分特化的 gate, 相較於 global memory 的速度有著更快的效能
% 其中, 在 量子運算的 gate fusion 階段中, 基礎 gate 只會被融合成這些特化的 gate.
% 在過往的研究中, fused-gate 正是因為這樣沒有保持運算的效率. (但 fused-gate 沒效率主要應該不是因為這些常數，而是過多的乘加運算，故不能任意 fuse)
% 我們所提出的解法，將有助於將模擬效能推往下一個階段
%Similar to rendering images, various types of gate operations, such as diagonal and unitary gate constants, can be stored in texture memory to reduce memory access and boost accessing bandwidth, enabling faster performance compared to GPU global memory.
%Similar to rendering images, there are multiple gate types requiring parameters, such as diagonal and unitary gates. By placing these parameters on texture memory specifically designed for constants, we achieve better performance compared to placing them on GPU global memory. This is because the load/store unit and texture unit are separated\cite{nsight_doc}. Since our workload heavily make use of load/store unit and the texture unit is mostly idle, by putting the parameters on the texture memory, we can reduce the use of load/store unit.
Similar to image rendering, certain types of gates, such as diagonal and unitary gates, necessitate read-only parameters.
Instead of relying solely on default global memory, we can maximize computational resources by placing these parameters on texture memory on modern GPU.
According to the NVIDIA Nsight Compute Documentation~\cite{nsight_doc}, the Load Store Unit (LSU) and Texture Unit (TEX) are designed in separate data pipelines.
Using global memory or constant memory alone may diminish overall DRAM bandwidth due to the occupancy of LSU.
Therefore, leveraging texture memory for constant variables presents a feasible alternative in quantum circuit simulation.
\end{comment}


%Given that our workload predominantly utilizes the load/store unit while the texture unit remains largely underused, allocating parameters to texture memory allows us to decrease reliance on the load/store unit, thereby improving overall efficiency.


\begin{comment}
Lines 7-11 of Algorithm~\ref{algo:simulation_flow} outline the core process for applying general gates. Each chunk is processed by a thread block. Before applying a gate block, the chunk's content is copied to shared memory. The gates within the block are then applied directly to the shared memory, minimizing data movement overhead. Finally, the updated chunk is copied back to global memory, completing the gate block application.
To improve the efficiency of quantum simulation, we employ several techniques:
\begin{enumerate}
    \item \textbf{Loop Unrolling:} Instead of assigning each thread to a single state, a thread handles 8 states. This reduces synchronization overhead, avoids redundant calculations, and minimizes access to constant values.
    \item \textbf{Shared Memory:} Shared memory acts as a user-managed cache significantly faster than global memory. By applying gates directly on shared memory, we achieve faster simulation speeds.
    \item \textbf{Texture Memory for Constants:} Our testing reveals that reading diagonal and unitary gate constants from texture memory surpasses global memory access in speed, though the exact reason for this advantage remains unclear.
\end{enumerate}
\end{comment}

%1. Decrease stall barrier: loop unrolling, lower sync operation
%2. Increase data locality: shared memory
%3. Increase access efficiency: texture memory

%A \emph{block-by-block} simulation scheme is proposed to accelerate quantum circuit simulations, which is called BlockQ. Two important aspects should be addressed toward BlockQ: partitioning quantum states into chunks and finding gate blocks so that the simulator can perform the updates on a subset of quantum states for as many quantum gates as possible, improving the data reuse and boosting the simulation performance. 

%\emph{\textbf{Partitioning quantum states into chunks}} enhances the data reuse for quantum state updates. As illustrated in \figurename~\ref{fig:simscheme}(b), a chunk-wise access pattern is adopted for the updates of quantum states to reflect the simulation effect for the three quantum gates. Specifically, the space reserved for quantum states is partitioned into four data chunks (as shown on the right of \figurename~\ref{fig:simscheme}(b)). During the simulation, the same data chunk is touched three times to update the quantum states for the three quantum gates. After the completion of the updates for the first chunk, the quantum states of the second chunk are loaded and updated, followed by the third and fourth chunks. This is referred to as a \emph{chunk-by-chunk} quantum state access pattern.

%The partitioning is done by introducing the concept of \emph{chunk bits}, which are the number of qubits $\mathcal{C}$ used for maintaining the $2^\mathcal{C}$ quantum states, which serve as the fundamental unit for facilitating quantum circuit simulation.
%When the quantum gates perform on these qubits, the required quantum states (i.e., pair of the qubits) are in the $2^\mathcal{C}$ quantum states\footnote{These partial quantum states are independent of other quantum states in some other chunks.}. By choosing a proper $\mathcal{C}$ value judiciously, a chunk can be retained in the processor cache (i.e., LLC) during the quantum state updates. 
%Furthermore, in scenarios where the target qubits $targs$ of consecutive gates all fall within the chunk bits (i.e., $targs \leq C$), the quantum states to be updated can be found within the same chunk, thereby eliminating redundant write accesses to the next level memory.

\begin{comment}
\subsection{Cache Line Characteristic}

\begin{algorithm}
    \caption{SQS Parameters Preparing}
    \label{alg:sqs_prepare}
    \SetKwInOut{KwInput}{Input}
    \SetKwInOut{KwOutput}{Output}

    \KwInput{$n$ is the number of qubits. $c$ is the cache line offset. $A$ and $B$ are sets containing the indices to the qubits that need to be swapped. $|A| = |B|$ and $ A \cap B = \varnothing$.}
    \KwOutput{Two sets, $P$ and $Q$. $|P| = |Q|$ and $P \cap Q = \varnothing$.}

    \BlankLine
    % Pseudocode start
    $A' \gets \{x \in A \mid x \le c \}$ \;
    $B' \gets \{x \in B \mid x \le c \}$ \;
    $d = | |A'| - |B'| |$\;
    $P \gets \{x \mid x \ge c \text{ and } x < c + d \ \text{ and } x < n\}$ \;
    \uIf{$a > b$}{
        $Q \gets $ $\{$$d$ smallest elements in $B - B'$$\}$ \;
    }\ElseIf{$a < b$}{
        $Q \gets $ $\{$$d$ smallest elements in $A - A'$$\}$ \;
    }
    $[P, Q] \gets [P - Q, Q - P]$ \;
    \Return {$P$, $Q$} \;
\end{algorithm}

\begin{algorithm}
    \caption{SQS algorithm for GPU}
    \SetKwInOut{KwInput}{Input}
    \SetKwInOut{KwOutput}{Output}

    \KwInput{$S$ is the state vector of quantum circuit simulation. $n$ is the number of qubits. $A$ and $B$ are sets containing the indices to the qubits that need to be swapped. $P$ and $Q$ are the result of the SQS parameters preparing algorithms. $|A| = |B|$ and $ A \cap B = \varnothing$. $|S| = 2^n$.}

    \KwOutput{$S$ is the state vector after qubits swapping.}

    \BlankLine

    % Function definitions
    \SetKwFunction{FbitSwap}{bitswap}
    \SetKwProg{Fn}{function}{:}{end}

    % Code Body
    \For{$t \gets 0$ \KwTo $2^n-1$} {
        $m \gets$ \FbitSwap($t$, $P$, $Q$) \;
        $n \gets$ \FbitSwap($m$, $A$, $B$) \;
        \If {$m < n$} {
            Swap $S[m]$ and $S[n]$ \;
        }
    }
    \BlankLine
    \Fn{\FbitSwap{$i$, $A$, $B$}} {
        \tcp{In this function, we use $i[n]$ to denote the $n^{th}$ bit of the integer $i$. $i[0]$ is the LSB.}
        \While{$A \neq \varnothing$} {
            Let $a$ and $b$ be the smallest integer in $A$ and $B$ \;
            Remove $a$ and $b$ in $A$ and $B$ \;
            Swap $i[a]$ and $i[b]$ \;
        }
        \Return $i$ as an integer
    }
    \BlankLine
\end{algorithm}
\end{comment}

\subsection{In-memory Swapping (IMS)}
\label{sec:sqs}
In our implementation of cache-aware quantum circuit simulation, one of the predominant factors driving overall performance improvement is qubit swapping between the cache and memory region.
%While the most naive approach involves employing either the native swap gate or the fused swap gate, these approaches necessitate an excessive number of swap gates, or the closure of numerous threads to guarantee correct simulation results.
%Consequently, the simulation time in a single rank is even worse than when these approaches are not used.
While the most naive approach is to employ either native swap gates or fused swap gates, this approach necessitates an excessive number of swap gates when there are many pairs of qubits that need to be swapped.

In-memory swapping (IMS) is proposed as a critical solution to swap all pairs of qubits once and for all. %without relying on specific libraries~\cite{cutt}.
To efficiently implement this swapping operation for GPUs, it is not sufficient to intuitively apply threads to locate the corresponding positions of states and perform the swap, due to a multitude of scattered memory accesses.
Contrarily, our IMS is designed to thoroughly utilize the characteristics of cache lines, which serve as the basic unit for transferring data between cache and memory, as detailed in Algorithm~\ref{algo:sqs}.

% -> explanation for algorithm.
The $2^N$ state vector can be parallelized by $2^N$ GPU threads, with a variable $t$ representing each thread ID in Line 1.
Then, the pair of cache-friendly indices $m$ and $n$ can be calculated by~\emph{bitshift()} and~\emph{bitswap()} functions in Lines 2-3.
The \emph{bitshift()} function shifts $c$ bits from the left of the most significant bit of $\mathit{CL}$ to the positions that match the lowest $c$ qubits being swapped in. Here, $c$ represents the number of swapped-out bits located within $\mathit{CL}$ offsets.
The \emph{bitswap()} function is the original mapping rule of quantum computing for the qubit swapping.
After this stage, \textit{stateVector} is swapped with these indices in Lines 4-6.

\figurename{~\ref{fig:sqs}} illustrates an example of the IMS process with the swapping out set \{${q_0, q_2, q_3, q_4, q_5}$\} and swapping in set \{${q_6, q_7, q_9, q_{10}, q_{11}}$\}.
In this case, $t_3$ and $t_4$ of each thread correspond to $q_6$ and $q_7$ of the original qubit representation.
Consequently, the swapping rule is used to map them to the swapped-out indices $q_0$ and $q_2$.
All bits of $m$ and $n$ that are in $\mathit{CL}$ must be mapped from the bits of thread block offsets (e.g., The indexes $t_0, ..., t_5$ of thread marked in red within \figurename{~\ref{fig:sqs}}), ensuring that each state in a cache line is accessed by the same thread block, and data brought into the cache can be fully utilized before they are evicted.
%The indexing bits of each thread, initially in $C$ and are now in $\mathit{CL}$, provide clear evidence for this optimization.

It is worth noting that our approaches can seamlessly transition to various systems and architectures to match specific CPUs, GPUs, and other brand-new accelerators, while also not relying on any external libraries~\cite{cutt}.

%In our quantum simulation framework, in-memory swapping plays a crucial role in preparing the state vector for the application of gate blocks. Before applying a gate block to a state vector, it is necessary to reorder all target qubits of the gate block into chunk offsets, which means that gate operations do not involve qubits across chunks. This reordering involves swapping indices of qubits within the state vector.

%The workflow for qubit swapping is detailed in Algorithm \ref{alg:sqs}. For each state with index $m$, the corresponding state with index $n$ is identified by swapping bits on $m$ based on the qubits to be swapped out and in. The states indexed as $m$ and $n$ are then swapped if $m > n$. This conditional check, $m > n$, ensures that each state requiring swapping is processed exactly once.

%To implement qubit swapping on a GPU, the loop at line 1 of Algorithm \ref{algo:sqs} can be parallelized with $2^n$ threads, where the thread ID of each thread is used as $m$. However, this parallelization approach lacks cache-friendliness because memory accesses to $S[n]$ at line 4 of Algorithm \ref{algo:sqs} are scattered when qubits being swapped out reside in the cache line offsets.
%An index calculation algorithm is proposed to enhance the cache-friendliness of qubit swapping. Instead of directly using the thread ID as $m$, this algorithm maps thread IDs to $m$ using the following calculation: Let $t$ be the thread ID, and $c$ be the number of qubits in the cache line offsets that are being swapped out. The index $m$ is obtained by shifting $c$ bits of $t$ from the left of the most significant bit of cache line offsets to the positions that match the lowest $c$ qubits being swapped in. 


%Fig. \ref{fig:sqs} is an example of how the index calculation works. The qubits being swapped out are 0, 2, 3, 4, 5 and the qubits being swapped in are 8, 9, 11, 12, 13. As illustrated in the figure, with the index calculation algorithm, bits that are in cache line offsets are mapped from the 5 lowest significant bits ($t_0 ... t_4$), which are within the thread block offsets. This ensures the full utilization of cache lines.
%After calculating the index $m$ using the above algorithm, Algorithm \ref{alg:sqs} can be continued to complete the qubit swapping process.

%After calculating the index $m$ using the above algorithm, Algorithm \ref{alg:sqs} can be continued to complete the qubit swapping process.

\begin{figure}[tb!]
%\centerline{\includegraphics[width=.95\columnwidth]{figures/sqs_index.pdf}}
\centerline{\includegraphics[width=.95\columnwidth]{figures/sqs.pdf}}
\caption{An example of the in-memory swapping process.
%The qubits in the golden region represent the swapped-out qubits, while those in the blue region represent the swapped-in qubits.
}
\label{fig:sqs}
\end{figure}

\begin{algorithm}
    \caption{Pseudo-code of in-memory swappipng}
    \label{algo:sqs}
    \SetKwInOut{KwInput}{Input}
    \SetKwInOut{KwOutput}{Output}

    %\KwInput{$S$ is a state vector representing an $n$-qubit quantum state. Set $A$ are indices of qubits out of chunk that will be swapped in. Set $B$ are indices of qubits in chunk that will be swapped out.}
    \KwInput{The indices of qubits that are swapped in the chunk ($A$) and swapped out of the chunk ($B$).
    }
    %, respectively.}
    %cl$ is the number of bits of cache line offset
    %\KwOutput{$S$ is the state vector after qubit swapping.}

    \For{$t \gets 0$ \KwTo $2^N - 1$} {
        %$clc \gets$ the number of qubits in $B$ that are in the cache line offsets\;
        %$m \gets$ Shift $c$ bits of $t$ from the left of the most significant bit of cache line offsets to the positions that match the lowest $c$ qubits being swapped in.
        $m$ $\gets$ bitshift($t$, $A$, $B$, $\mathit{CL}$) \\
        $n$ $\gets$ bitswap($m$, $A$, $B$) \\
        \If {$m > n$} {
            %Swap $S[m]$ and $S[n]$ \;
            swap($\textit{stateVector}[m]$, $\textit{stateVector}[n]$) \\
        }
    }
    
\end{algorithm}

%Let $c$ be the number of qubits of $B$ that are in cache line offsets \;
%$m \gets $ The result of shifting $c$ bits of $t$ starting from the $3^{\text{rd}}$ bit to the indices of $c$ smallest qubits in $A$ \;
